The Gateaux Derivative and Integral over Banach Algebra

In the paper I considered definition and structure of linear mapping of Banach algebra over commutative ring. Based on this definition I explore derivative of continuous mapping.

==> Abstract.1006.2597.Russian.tex <==
%auto-ignore
\def\P{\partial}
\def\S{\sum_{n=0}^{\infty}(n!)^{-1}}
\def\G{Гато\ }
\def\M{$f:A\rightarrow A\ $}
Пусть $A$ - алгебра над коммутативным кольцом $D$. Отображение
\M
линейно, если для любых $a,b\in A$ и любого $c\in D$
\[
f\circ (a+b)=f\circ a+f\circ b
\]
\[
f\circ(ca)=c\ f\circ a
\]
Функция
\M
дифференцируема по Гато,
если
\[
f(x+a)-f(x)
=\P f(x)\circ a
+o(a)
\]
где
производная \G
$\P f(x)$
отображения $f$
- линейное отображение приращения $a$ и
$o$ - такое непрерывное отображение, что
\[
\lim_{a\rightarrow 0}\frac{|o(a)|}{|a|}=0
\]
Например
\[
\P (x^2)\circ h=xh+hx
\]
\[
\P (x^{-1})\circ h=-x^{-1}hx^{-1}
\]

Предполагая, что определена производная \G
$\P^{n-1} f(x)$ порядка $n-1$, мы определим
\[
\P^n f(x)\circ(a_1\otimes...\otimes a_n)
=\P(\P^{n-1} f(x)\circ(a_1\otimes...\otimes a_{n-1}))\circ a_n
\]
производную \G порядка $n$ отображения $f$.
Если $h_1=...=h_n=h$, то мы положим
\[
\P^nf(x)\circ h=\P^nf(x)\circ(h_1\otimes...\otimes h_n)
\]

Функция $f(x)$ имеет разложение в ряд Тейлора
\[
f(x)=\S\P^n f(x_0)\circ(x-x_0)
\]

Дифференциальное уравнение над телом
\[
\P (y)\circ h=hx^2+xhx+x^2h
\]
\[
y(0)=0
\]
имеет решение
\[
y=x^3
\]

Решением дифференциального уравнения
\[
\P(y)\circ h=\frac 12(yh+hy)
\]
\[y(0)=1\]
является экспонента
$y=e^x$
которая имеет следующее разложение в ряд Тейлора
\[
e^x=\S x^n
\]
Равенство
\[
e^{a+b}=e^ae^b
\]
справедливо тогда и только тогда, когда
$ab=ba$



==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Mappings of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
При этом подразумевается, что отображение мультипликативно над
максимально возможным полем. В частности, линейное отображение
тела $D$ мультипликативно над центром $Z(D)$. Это не противоречит
определению линейного отображения поля, так как для поля $F$ справедливо
$Z(F)=F$.
Если поле $F$ отлично
от максимально возможного, то я это явно указываю в тексте.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - свободная конечно
мерная алгебра.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
Однако в алгебре не принято использовать векторные обозначения.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}

\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Derivative.Russian.tex <==
%auto-ignore

\input{\FilePrefix Derivative.Eq}

\Chapter{Дифференцируемые отображения}
\label{chapter: Differentiable maps}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
В этом разделе мы изучим производную и дифференциал отображения
в $D$\hyph алгебру.
Поле комплексных чисел - это алгебра над полем действительных чисел.
В математическом анализе функций комплексного переменного мы рассматриваем
линейные отображения, порождённые отображением $I_0\circ z=z$.
Поэтому и в этом разделе мы ограничимся линейными отображениями, порождёнными
отображением $I_0\circ a=a$.
\fi%Calculus.Paper

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\Section{Топологическое кольцо}
\label{section: Topological Ring}

\begin{definition}
Кольцо $D$ называется 
\AddIndex{топологическим кольцом}{topological ring}\footnote{Определение
дано согласно
определению из \citeBib{Pontryagin: Topological Group},
глава 4},
если $D$ является топологическим пространством, и алгебраические операции,
определённые в $D$, непрерывны в топологическом пространстве $D$.
\qed
\end{definition}

Согласно определению, для произвольных элементов $a$, $b\in D$
и для произвольных окрестностей $W_{a-b}$ элемента $a-b$,
$W_{ab}$ элемента $ab$ существуют такие окрестности $W_a$
элемента $a$ и $W_b$ элемента $b$, что $W_a-W_b\subset W_{a-b}$,
$W_aW_b\subset W_{ab}$.

\begin{definition}
\label{definition: norm on ring}
\AddIndex{Норма на кольце}
{norm on ring} $D$\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2, а также согласно
определению \citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.} - это отображение
\[d\in D\rightarrow |d|\in R\]
такое, что
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ равносильно $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Кольцо $D$, наделённое структурой, определяемой заданием на
$D$ нормы, называется
\AddIndex{нормированным кольцом}{normed ring}.
\qed
\end{definition}

Инвариантное расстояние на аддитивной группе кольца $D$
\[d(a,b)=|a-b|\]
определяет топологию метрического пространства,
согласующуюся со структурой кольца в $D$.

\begin{definition}
\label{definition: limit of sequence, normed ring}
Пусть $D$ - нормированное кольцо.
Элемент $a\in D$ называется 
\AddIndex{пределом последовательности}{limit of sequence, normed ring}
\ShowEq{limit of sequence, normed ring}
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon$ для любого $n>n_0$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: limit of sequence, normed ring, product on scalar}
Пусть $D$ - нормированное кольцо характеристики $0$ и пусть $d\in D$.
Пусть $a\in D$ - предел последовательности $\{a_n\}$.
Тогда
\[
\lim_{n\rightarrow\infty}(a_nd)=ad
\]
\[
\lim_{n\rightarrow\infty}(da_n)=da
\]
\end{theorem}
\begin{proof}
Утверждение теоремы тривиально, однако я привожу доказательство
для полноты текста. 
Поскольку $a\in D$ - предел последовательности $\{a_n\}$,
то согласно определению
\ref{definition: limit of sequence, normed ring}
для заданного $\epsilon\in R$, $\epsilon>0$,
существует натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon/|d|$ для любого $n>n_0$.
Согласно определению \ref{definition: norm on ring}
утверждение теоремы следует из неравенств
\[
|a_nd-ad|=|(a_n-a)d|=|a_n-a||d|<\epsilon/|d||d|=\epsilon
\]
\[
|da_n-da|=|d(a_n-a)|=|d||a_n-a|<|d|\epsilon/|d|=\epsilon
\]
для любого $n>n_0$.
\end{proof}

\begin{definition}
Пусть $D$ - нормированное кольцо.
Последовательность $\{a_n\}$, $a_n\in D$ называется 
\AddIndex{фундаментальной}{fundamental sequence, normed ring}
или \AddIndex{последовательностью Коши}{Cauchy sequence, normed ring},
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $ \epsilon$, натуральное число $n_0$ такое,
что $|a_p-a_q|<\epsilon$ для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированное кольцо $D$ называется 
\AddIndex{полным}{complete ring}
если любая фундаментальная последовательность элементов
данного кольца сходится, т. е.
имеет предел в этом кольце.
\qed
\end{definition}

В дальнейшем, говоря о нормированном кольце характеристики $0$,
мы будем предполагать, что определён гомеоморфизм поля рациональных
чисел $Q$ в кольцо $D$.

\begin{theorem}
\label{theorem: complete ring contains real number}
Полное кольцо $D$ характеристики $0$
содержит в качестве подполя изоморфный образ поля $R$
действительных чисел.
Это поле обычно отождествляют с $R$.
\end{theorem}
\begin{proof}
Рассмотрим фундаментальную последовательность рациональных чисел $\{p_n\}$.
Пусть $p'$ - предел этой последовательности в теле $D$.
Пусть $p$ - предел этой последовательности в поле $R$.
Так как вложение поля $Q$ в тело $D$ гомеоморфно,
то мы можем отождествить $p'\in D$ и $p\in R$.
\end{proof}

\begin{theorem}
\label{theorem: complete ring and real number}
Пусть $D$ - полное кольцо характеристики $0$ и пусть $d\in D$.
Тогда любое действительное число $p\in R$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить действительное число $p\in R$ в
виде фундаментальной последовательности рациональных чисел $\{p_n\}$.
Утверждение теоремы следует из цепочки равенств
\[
pd=\lim_{n\rightarrow\infty}(p_nd)=\lim_{n\rightarrow\infty}(dp_n)=dp
\]
основанной на утверждении теоремы
\ref{theorem: limit of sequence, normed ring, product on scalar}.
\end{proof}

\Section{Топологическая \texorpdfstring{$D$}{D}-алгебра}

\begin{definition}
Пусть $D$ - топологическое коммутативное кольцо.
$D$\Hyph алгебра $A$ называется 
\AddIndex{топологической $D$\Hyph алгеброй}
{topological D algebra}\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: Topological Vector Space},
с. 21},
если $A$ наделено топологией, согласующейся со
структурой аддитивной группы в $A$,
и отображения
\ShowEq{topological D algebra}
непрерывны.
\qed
\end{definition}

\begin{definition}
\label{definition: norm on d algebra}
\AddIndex{Норма на $D$\Hyph алгебре}
{norm on D algebra} $A$
над нормированым коммутативным кольцом $D$\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$3} - это отображение
\ShowEq{norm on d algebra}
такое, что
\begin{itemize}
\ShowEq{norm on d algebra 1}
\ShowEq{norm on d algebra 2, 1}
равносильно
\ShowEq{norm on d algebra 2, 2}
\ShowEq{norm on d algebra 3}
\end{itemize}

$D$\Hyph алгебра $A$
над нормированным коммутативным кольцом $D$,
наделённая структурой, определяемой заданием на
$A$ нормы, называется
\AddIndex{нормированной $D$\Hyph алгеброй}{normed D algebra}.
\qed
\end{definition}

\begin{definition}
\label{definition: limit of sequence, normed algebra}
Пусть $A$ - нормированная $D$\Hyph алгебра.
Элемент $a\in A$ называется 
\AddIndex{пределом последовательности}{limit of sequence, normed algebra}
\ShowEq{limit of sequence, normed algebra}
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon$ для любого $n>n_0$.
\qed
\end{definition}

\begin{definition}
Пусть $A$ - нормированная $D$\Hyph алгебра.
Последовательность $\{a_n\}$, $a_n\in A$ называется 
\AddIndex{фундаментальной}{fundamental sequence, normed algebra}
или \AddIndex{последовательностью Коши}{Cauchy sequence, normed algebra},
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $ \epsilon$, натуральное число $n_0$ такое,
что $|a_p-a_q|<\epsilon$ для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированная $D$\Hyph алгебра $A$ называется 
\AddIndex{банаховой $D$\Hyph алгеброй}{Banach algebra}
если любая фундаментальная последовательность элементов
алгебры $A$ сходится, т. е.
имеет предел в алгебре $A$.
\qed
\end{definition}

\begin{definition}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Множество элементов
\ShowEq{unit sphere in algebra}
называется
\AddIndex{единичной сферой в алгебре}{unit sphere in algebra} $A$.
\qed
\end{definition}

\begin{definition}
\label{definition: continuous function, algebra}
Отображение
\ShowEq{f A1 A2}
банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$
называется \AddIndex{непрерывной}{continuous function, algebra}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{definition}
\label{definition: norm of map, algebra}
Пусть
\ShowEq{f A1 A2}
отображение банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$.
Величина
\ShowEq{norm of map, algebra}
называется
\AddIndex{нормой отображения $f$}
{norm of map, algebra}.
\qed
\end{definition}

\begin{theorem}
Пусть
\ShowEq{f A1 A2}
линейное отображение банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$.
Тогда
\ShowEq{norm of linear map, algebra}
\end{theorem}
\begin{proof}
Из определения
\ref{definition: linear map from A1 to A2, algebra}
и теоремы
\ref{theorem: complete ring contains real number}
следует
\ShowEq{linear map and real number}
Из равенства \EqRef{linear map and real number}
и определения \ref{definition: norm on d algebra}
следует
\ShowEq{linear map and real number, 1}
Полагая $\displaystyle r=\frac 1{|x|_1}$, мы получим
\ShowEq{norm of linear map, algebra, 1}
Равенство \EqRef{norm of linear map, algebra}
следует из равенств \EqRef{norm of linear map, algebra, 1}
и \EqRef{norm of map, algebra}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{f A1 A2}
линейное отображение банаховой $D_1$\Hyph алгебры $A_1$ с нормой $|x|_1$
в банаховую $D_2$\Hyph алгебру $A_2$ с нормой $|y|_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ линейно, то
согласно определению \ref{definition: norm of map, algebra}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous function, algebra}
отображение $f$ непрерывно.
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: continuity of map, norm, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
отображение полного тела $D_1$
в полное тело $D_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ аддитивно, то
согласно определению \ref{definition: norm of map, algebra}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous function, algebra}
отображение $f$ непрерывно.
\end{proof}
\fi
\else
\newpage
\fi

\Section{Производная отображений алгебры}
\label{section: The Derivative of Mapping in Algebra}

\begin{definition}
\label{definition: function differentiable in Gateaux sense, algebra}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Функция
\ShowEq{f:A->A}
\AddIndex{дифференцируема по Гато}
{function differentiable in Gateaux sense, algebra}
на множестве $U\subset A$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\ShowEq{Gateaux derivative of map, algebra}
где
\AddIndex{производная Гато
$\ShowSymbol{Gateaux derivative of map, algebra}$
отображения $f$}
{Gateaux derivative of map, algebra}
- линейное отображение приращения $a$ и
\ShowEq{Gateaux derivative of map, algebra, 1}
- такое непрерывное отображение, что
\ShowEq{Gateaux derivative of map, algebra, 2}
\qed
\end{definition}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{remark}
\label{remark: differential L(A,A)}
Согласно определению
\ref{definition: function differentiable in Gateaux sense, algebra}
при заданном $x$ производная Гато
\ShowEq{differential L(A,A), 1}
Следовательно, производная Гато отображения $f$ является отображением
\ShowEq{differential L(A,A), 2}
Выражения $\partial f(x)$ и $\displaystyle\frac{\partial f(x)}{\partial x}$
являются разными обозначениями одной и той же функции.
Мы будем пользоваться обозначением $\displaystyle\frac{\partial f(x)}{\partial x}$,
если хотим подчеркнуть, что мы берём производную Гато по переменной $x$.
\qed
\end{remark}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{theorem}
\label{theorem: function differentiable in Gateaux sense, algebra}
Мы можем представить \AddIndex{дифференциал Гато
\ShowEq{Gateaux differential of map, algebra}
отображения $f$}
{Gateaux differential of map, algebra}
в виде\footnote{Формально, мы должны записать дифференциал отображения в виде
\ShowEq{Gateaux differential, representation, algebra, 1}
Однако, например, в теории функций комплексного переменного рассматриваются
только линейные отображения, порождённые отображением $I_0\circ z=z$.
Поэтому при изучении производных мы также ограничимся
линейные отображениями, порождёнными отображением $I_0$.
Переход к общему случаю не составляет особого труда.
}
\ShowEq{Gateaux differential, representation, algebra}
Выражение
\ShowEq{component of Gateaux derivative of map, algebra}
называется
\AddIndex{компонентой производной Гато отображения $f(x)$}
{component of Gateaux derivative of map, algebra}.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: function differentiable in Gateaux sense, algebra}
и теоремы
\ref{theorem: linear mapping in L(A,A), associative algebra}.
\end{proof}

Из определений
\ref{definition: linear map from A1 to A2, algebra},
\ref{definition: function differentiable in Gateaux sense, algebra}
и теоремы
\ref{theorem: complete ring contains real number}
следует
\ShowEq{Gateaux differential is multiplicative over field R, algebra}
Комбинируя равенство
\EqRef{Gateaux differential is multiplicative over field R, algebra}
и определение
\ref{definition: function differentiable in Gateaux sense, algebra},
мы получим знакомое определение дифференциала
Гато
\ShowEq{Gateaux differential, representation in algebra}
Определения производной Гато
\EqRef{Gateaux derivative of map, algebra}
и \EqRef{Gateaux differential, representation in algebra}
эквивалентны. На основе этой эквивалентности мы будем говорить,
что отображение $f$
дифференцируемо по Гато на множестве $U\subset D$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\ShowEq{Gateaux differential of map, t, algebra}
где
$o:R\rightarrow A$ - такое непрерывное отображение, что
\[
\lim_{t\rightarrow 0}\frac{|o(t)|}{|t|}=0
\]
\fi

\begin{theorem}
\label{theorem: Gateaux differential, standard form, algebra}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
\AddIndex{Стандартное представление производной Гато отображения}
{Gateaux derivative, standard representation, algebra}
\ShowEq{f:A->A}
имеет вид
\ShowEq{Gateaux derivative, algebra, standard representation}
Выражение
\ShowEq{standard component of Gateaux derivative, algebra}
в равенстве
\EqRef{Gateaux derivative, algebra, standard representation}
называется
\AddIndex{стандартной компонентой производной Гато отображения $f$}
{standard component of Gateaux derivative, algebra}.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием
утверждения \eqref{f in L(A,A), 2, associative algebra} теоремы
\ref{theorem: linear mapping in L(A,A), associative algebra}.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential and jacobian, algebra}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть $\Basis e$ - алгебры $A$ над кольцом $D$.
Тогда дифференциал Гато отображения
\[
f:D\rightarrow D
\]
можно записать в виде
\ShowEq{Gateaux differential and jacobian, algebra}
где $dx\in A$ имеет разложение
\ShowEq{Gateaux differential and jacobian, 1, algebra}
относительно базиса $\Basis e$ и матрица Якоби отображения $f$ имеет вид
\ShowEq{standard components and Jacobian, algebra}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ref{theorem: linear mapping in L(A,A), associative algebra}.
\end{proof}

\begin{theorem}
\label{theorem: derivative of the sum}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{bilinear map and derivative, 1}
Отображение
\ShowEq{derivative of the sum, 2}
дифференцируемо и
производная Гато удовлетворяет соотношению
\ShowEq{derivative of the sum, 3}
\end{theorem}
\begin{proof}
Согласно определению
\EqRef{Gateaux differential, representation in algebra},
\ShowEq{derivative of the sum, 4}
Равенство \EqRef{derivative of the sum, 3}
следует из равенства \EqRef{derivative of the sum, 4}.
\end{proof}

\begin{theorem}
\label{theorem: bilinear map and derivative}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть
\ShowEq{bilinear map and derivative}
непрерывное билинейное отображение.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{bilinear map and derivative, 1}
Отображение
\ShowEq{bilinear map and derivative, 2}
дифференцируемо и
дифференциал Гато удовлетворяет соотношению
\ShowEq{bilinear map and derivative, 3}
\end{theorem}
\begin{proof}
Равенство \EqRef{bilinear map and derivative, 3}
следует из цепочки равенств
\ShowEq{bilinear map and derivative, 4}
основанной на определении
\EqRef{Gateaux differential, representation in algebra}.
\end{proof}
\fi

\begin{theorem}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть $f$, $g$ - дифференцируемые отображения
\ShowEq{bilinear map and derivative, 1}
Дифференциал Гато удовлетворяет соотношению
\ShowEq{Gateaux differential of product, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
{\bf Таблица производных отображений ассоциативной алгебры}
\else
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: bilinear map and derivative}
и определения \ref{definition: algebra over ring}.
\end{proof}

\begin{theorem}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Допустим производная Гато отображения
\ShowEq{f:A->A}
имеет разложение
\ShowEq{Gateaux derivative of f, algebra}
Допустим производная Гато отображения
$g:D\rightarrow D$
имеет разложение
\ShowEq{Gateaux derivative of g, algebra}
Производная Гато отображения $f(x)g(x)$
имеет вид
\ShowEq{Gateaux derivative, fg, algebra}
\end{theorem}
\begin{proof}
Подставим \EqRef{Gateaux derivative of f, algebra}
и \EqRef{Gateaux derivative of g, algebra}
в равенство \EqRef{Gateaux differential of product, algebra}
\begin{align}
\EqLabel{Gateaux differential of fg, division ring}
\partial (f(x) g(x))(a)
&=\partial f(x)(a)\ g(x)+f(x)\ \partial g(x)(a)
\\ \nonumber
&=\frac{\pC{s}{0}\partial f(x)}{\partial x}a
\frac{\pC{s}{1}\partial f(x)}{\partial x}
g(x)
+f(x)\frac{\pC{t}{0}\partial g(x)}{\partial x}a
\frac{\pC{t}{1}\partial g(x)}{\partial x}
\end{align}
Опираясь на \EqRef{Gateaux differential of fg, division ring},
мы определяем равенства
\EqRef{0 component of Gateaux derivative, fg, algebra},
\EqRef{1 component of Gateaux derivative, fg, algebra}.
\end{proof}

\begin{theorem}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Если производная Гато
$\partial f(x)$
существует в точке $x$ и имеет конечную норму,
то отображение $f$ непрерывно в точке $x$.
\end{theorem}
\begin{proof}
Из определения \ref{definition: norm of map, algebra}
следует
\ShowEq{derivative and continuos function, algebra, 1}
Из \EqRef{Gateaux derivative of map, algebra},
\EqRef{derivative and continuos function, algebra, 1}
следует
\begin{equation}
\EqLabel{derivative and continuos function, algebra, 2}
|f(x+a)-f(x)|<|a|\ \|\partial f(x)\|
\end{equation}
Возьмём произвольное $\epsilon>0$. Положим
\[\delta=\frac\epsilon{\|\partial f(x)\|}\]
Тогда из неравенства
\[
|a|<\delta
\]
следует
\[
|f(x+a)-f(x)|\le \|\partial f(x)\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous function, algebra}
отображение $f$ непрерывно в точке $x$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative, 0, D algebra}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть отображение
\ShowEq{f:A->A}
дифференцируемо по Гато в точке
$x$.
Тогда
\ShowEq{Gateaux derivative, 0, D algebra}
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: function differentiable in Gateaux sense, algebra}
и теоремы
\ref{theorem: linear map, 0, D algebra}.
\end{proof}

\begin{theorem}
\label{theorem: composite map, derivative, D algebra}
Пусть $A$ - банаховая $D$\Hyph алгебра.
Пусть отображение
\ShowEq{f:A->A}
дифференцируемо по Гато в точке
$x$
и норма производной Гато отображения $f$
конечна
\ShowEq{composite map, norm f, D algebra}
Пусть отображение
\ShowEq{g:A->A}
дифференцируемо по Гато в точке
\ShowEq{composite map, y fx, D algebra}
и норма производной Гато отображения $g$
конечна
\ShowEq{composite map, norm g, D algebra}
Отображение
\ShowEq{composite map, gfx, D algebra}
дифференцируемо по Гато в точке
$x$
\ShowEq{composite map, derivative, D algebra}
\ShowEq{composite map, Gateaux derivative 01, D algebra}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: function differentiable in Gateaux sense, algebra}
\ShowEq{Gateaux derivative of map g, D algebra}
где
\ShowEq{o1:A->A}
- такое непрерывное отображение, что
\ShowEq{o1:A->A, 1}
Согласно определению
\ref{definition: function differentiable in Gateaux sense, algebra}
\ShowEq{Gateaux derivative of map f, D algebra}
где
\ShowEq{o2:A->A}
- такое непрерывное отображение, что
\ShowEq{o2:A->A, 1}
Согласно
\EqRef{Gateaux derivative of map f, D algebra}
смещение $a$ значения $x\in A$
приводит к смещению
\ShowEq{composite map, b fxa, D algebra}
значения $y$.
Используя \EqRef{composite map, y fx, D algebra},
\EqRef{composite map, b fxa, D algebra}
в равенстве \EqRef{Gateaux derivative of map g, D algebra},
мы получим
\ShowEq{Gateaux derivative of map gf, 1, D algebra}
Согласно определениям
\ref{definition: function differentiable in Gateaux sense, algebra},
\ref{definition: linear map from A1 to A2, algebra}
из равенства \EqRef{Gateaux derivative of map gf, 1, D algebra}
следует
\ShowEq{Gateaux derivative of map gf, 2, D algebra}
Согласно определению \ref{definition: norm on d algebra}
\ShowEq{Gateaux derivative of map gf, 3, D algebra}
Из \EqRef{composite map, norm g, D algebra}
следует
\ShowEq{Gateaux derivative of map gf, 4, D algebra}
Из \EqRef{composite map, norm f, D algebra}
следует
\ShowEq{Gateaux derivative of map gf, 6, D algebra}
Согласно теореме \ref{theorem: Gateaux derivative, 0, D algebra}
\ShowEq{Gateaux derivative of map gf, 7, D algebra}
Следовательно,
\ShowEq{Gateaux derivative of map gf, 5, D algebra}
Из равенств
\EqRef{Gateaux derivative of map gf, 3, D algebra},
\EqRef{Gateaux derivative of map gf, 4, D algebra},
\EqRef{Gateaux derivative of map gf, 5, D algebra}
следует
\ShowEq{Gateaux derivative of map gf, 8, D algebra}
Согласно определению
\ref{definition: function differentiable in Gateaux sense, algebra}
\ShowEq{Gateaux derivative of map gf, 9, D algebra}
где
\ShowEq{Gateaux derivative of map, algebra, 1}
- такое непрерывное отображение, что
\ShowEq{Gateaux derivative of map, algebra, 2}
Равенство \EqRef{composite map, derivative, D algebra}
следует из
\EqRef{Gateaux derivative of map gf, 2, D algebra},
\EqRef{Gateaux derivative of map gf, 8, D algebra},
\EqRef{Gateaux derivative of map gf, 9, D algebra}.

Из равенства \EqRef{composite map, derivative, D algebra}
и теоремы
\ref{theorem: function differentiable in Gateaux sense, algebra}
следует
\ShowEq{composite map, derivative 2, D algebra}
\EqRef{composite map, Gateaux derivative 01, D algebra}
следуют из равенства
\EqRef{composite map, derivative 2, D algebra}.
\end{proof}
\fi

\Section{Таблица производных отображений ассоциативной алгебры}

\begin{theorem}
\label{theorem: Gateaux derivative of const, algebra}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда для любого $b\in A$
\ShowEq{Gateaux derivative of const, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Непосредственное следствие определения
\ref{definition: function differentiable in Gateaux sense, algebra}.
\end{proof}
\fi

\begin{theorem}
\label{theorem: Gateaux derivative, product over constant, algebra}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда для любых $b$, $c\in A$
\ShowEq{Gateaux derivative, product over constant, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Непосредственное следствие равенств
\EqRef{Gateaux differential of product, algebra},
\EqRef{0 component of Gateaux derivative, fg, algebra},
\EqRef{1 component of Gateaux derivative, fg, algebra},
так как $\partial b=\partial c=0$.
\end{proof}
\fi

\begin{theorem}
\label{theorem: Gateaux derivative, fx=axb, algebra}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда для любых $b$, $c\in A$
\ShowEq{Gateaux derivative, fx=axb, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Gateaux derivative, product over constant, algebra},
когда $f(x)=x$.
\end{proof}
\fi

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: Gateaux derivative of linear map}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Пусть $f$ - линейное отображение
\ShowEq{derivative linear map associative algebra}
Тогда
\ShowEq{derivative linear map associative algebra, 1}
\end{theorem}
\begin{proof}
Следствие теорем
\ref{theorem: Gateaux derivative, fx=axb, algebra},
\ref{theorem: derivative of the sum}.
\end{proof}
\fi

\begin{corollary}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда для любого $b\in A$
\ShowEq{Gateaux derivative, xb-bx, algebra}
\qed
\end{corollary}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{theorem}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Тогда\footnote{Утверждение теоремы аналогично примеру VIII,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\EqRef{derivative x2, algebra}
принимает вид
\ShowEq{derivative x2, field}}
\ShowEq{derivative x2, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Рассмотрим приращение функции $f(x)=x^2$.
\ShowEq{derivative x2, algebra, 1}
\EqRef{derivative x2, algebra}
следует из равенств \EqRef{Gateaux differential, representation, algebra},
\EqRef{derivative x2, algebra, 1}.
\end{proof}
\fi

\begin{theorem}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Тогда\footnote{Утверждение теоремы аналогично примеру IX,
\citeBib{Hamilton Elements of Quaternions 1}, с. 451.
Если произведение коммутативно, то равенство
\EqRef{derivative x power -1, algebra}
принимает вид
\ShowEq{derivative x power -1, field}}
\ShowEq{derivative x power -1, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Подставим $f(x)=x^{-1}$ в определение
\EqRef{Gateaux differential, representation in algebra}.
\ShowEq{derivative x power -1, algebra, 1}
Равенство \EqRef{derivative x power -1, algebra}
следует из цепочки равенств
\EqRef{derivative x power -1, algebra, 1}.
\end{proof}
\fi

\begin{theorem}
Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра с делением.
Тогда\footnote{Если произведение коммутативно, то
\[
y=xax^{-1}=a
\]
Соответственно производная обращается в $0$.}
\ShowEq{derivative xax power -1, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Равенство \EqRef{derivative xax power -1, algebra}
является следствием равенств
\EqRef{Gateaux differential of product, algebra},
\EqRef{Gateaux derivative, fx=axb, algebra}.
\end{proof}
\fi


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-rcd форма
   {$1$-\rcd форма}%
   {1-rcd form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%3%A%a b-CR квазидетерминант
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index%668%A%A CRcirc- базис модуля
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Index%667%A%A CRcirc- линейно ависимое множество векторов
   {$A\CRcirc$\Hyph линейно зависимое множество векторов}%
   {CRcirc linearly dependent, Astar module over algebra}%
\Index%666%A%A CRcirc- линейно независимое множество векторов
   {$A\CRcirc$\Hyph линейно независимое множество векторов}%
   {CRcirc linearly independent, Astar module over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc линейная комбинация
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination}%
\Index%581%A%Arc  линейно зависимые векторы
   {$A\RCstar$\Hyph  линейно зависимые векторы}%
   {linearly dependent, A vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%580%A%Arc линейно независимые векторы
   {$A\RCstar$\Hyph линейно независимые векторы}%
   {linearly independent, A vector space}%
\Index%789%A%Astar антилинейное отображение алгебры с сопряжением
   {$A\star$\Hyph антилинейное отображение алгебры с сопряжением}%
   {antilinear mapping of algebra with conjugation}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\Index%649%C%стандартная компонента полилинейного отображения в ассоциативную алгебру
   {стандартная компонента полилинейного отображения в ассоциативную алгебру}%
   {standard component of polylinear map, associative algebra}%
\SetIndexSpace%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%16%D%drc базис векторного пространства r строк
   {\drc базис векторного пространства \subs строк}%
   {drc basis, r rows vector space}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%30%D%drc вектор-функция
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%779%D%Dstar антилинейное отображение кольца с сопряжением
   {$D\star$\Hyph антилинейное отображение кольца с сопряжением}%
   {antilinear mapping of ring with conjugation}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%734%D%Dstar аффинное пространство
   {$D\star$\Hyph аффинное пространство}%
   {Dstar affine space}%
\Index%659%D%Dstar- базис модуля
   {$D\star$\Hyph базис модуля}%
   {D basis, module}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%658%D%Dstar линейно зависимые векторы Dstar модуля
   {$D\star$\Hyph линейно зависимые векторы $D\star$\Hyph модуля}%
   {Dstar linearly dependent, module}%
\Index%657%D%Dstar линейно независимые векторы Dstar модуля
   {$D\star$\Hyph линейно независимые векторы $D\star$\Hyph модуля}%
   {Dstar linearly independent, module}%
\Index%769%D%Dstar линейный гомоморфизм
   {$D\star$\Hyph линейный гомоморфизм}%
   {Dstar linear homomorphism}%
\Index%71%D%Dstar- модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%25%D%rcd базис в векторном пространстве c строк
   {\rcd базис в векторном пространстве \sups строк}%
   {rcd basis, c rows vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%49%R%drc базис, дуальный rcd базису в векторном пространстве
   {\drc базис, дуальный \rcd базису в векторном пространстве}%
   {basis dual to basis, rcd vector space}%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главный минор
   {\RC главный минор}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%677%R%RCcirc A- базис модуля
   {$\RCcirc A$\Hyph базис модуля}%
   {RCcirc A basis, module over algebra}%
\Index%676%R%RCcirc A- линейно ависимое множество векторов
   {$\RCcirc A$\Hyph линейно зависимое множество векторов}%
   {RCcirc linearly dependent, starA module over algebra}%
\Index%675%R%RCcirc A- линейно независимое множество векторов
   {$\RCcirc A$\Hyph линейно независимое множество векторов}%
   {RCcirc linearly independent, starA module over algebra}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%765%R%RCcircA линейная комбинация
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination}%
\Index%21%R%rcd  линейно зависимые векторы
   {\rcd  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%758%R%rcd аффинное преобразование
   {\rcd аффинное преобразование}%
   {rcd affine transformation}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%24%R%rcd базис в векторном пространстве
   {\rcd базис в векторном пространстве}%
   {rcd basis, vector space}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%34%R%rcd линейно независимые векторы
   {\rcd линейно независимые векторы}%
   {linearly independent, vector space}%
\Index%35%R%rcd линейное отображение векторных пространств
   {\rcd линейное отображение векторных пространств}%
   {rcd linear map of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%77%S%Dstar- произведением rcd линейного отображения A на скаляр
   {$D\star$\Hyph произведением \rcd линейного отображения $A$ на скаляр}%
   {Dstar product of rcd linear map over scalar}%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%683%S%star A- произведение Acr линейного отображения на скаляр
   {$\star A$\Hyph произведение \Acr линейного отображения на скаляр}%
   {starA product of Acr linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%88%T%Tstar- линейная комбинация векторов
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%616%А%ассоциатор R алгебры
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%689%Б%базис A- модуля
   {базис $A$\Hyph модуля}%
   {basis of A module}%
\Index%766%Б%базис ACRcirc модуля
   {базис $A\CRcirc$\Hyph модуля}%
   {basis of ACRcirc module}%
\Index%767%Б%базис CRcircA модуля
   {базис $\RCcirc A$\Hyph модуля}%
   {basis of CRcircA module}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%117%Б%базовый вектор представления группы Ли
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%782%В%вектор отображения
   {вектор отображения}%
   {vector of mapping}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%811%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное линейное отображение D- векторного пространства
   {вырожденное линейное отображение $D$\Hyph векторного пространства}%
   {singular linear map, D vector space}%
\Index%131%В%вырожденное линейное отображение тела
   {вырожденное линейное отображение тела}%
   {singular linear map, division ring}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%799%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%156%Д%дифференциал Гато второго порядка отображения \Vector f
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index%155%Д%дифференциал Гато второго порядка отображения f
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index%632%Д%дифференциал Гато второго порядка отображения f алгебры
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Index%157%Д%дифференциал Гато отображения \Vector f нормированного D- векторного пространства V в нормированное D- векторное пространство W
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index%158%Д%дифференциал Гато отображения f
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index%628%Д%дифференциал Гато отображения алгебры
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%809%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%654%З%закон ассоциативности для Dstar- модуля
   {закон ассоциативности для $D\star$\Hyph модуля}%
   {associative law, Dstar module}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%655%З%закон дистрибутивности для Dstar- модуля
   {закон дистрибутивности для $D\star$\Hyph модуля}%
   {distributive law, Dstar module}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%656%З%закон унитарности для Dstar- модуля
   {закон унитарности для $D\star$\Hyph модуля}%
   {unitarity law, Dstar module}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\SetIndexSpace%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%810%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%800%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор R алгебры
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%192%К%компонента линейного отображения D- векторного пространчства
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index%193%К%компонента линейного отображения f тела
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index%194%К%компонента полилинейного отображения \Vector A
   {компонента полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index%647%К%компонента полилинейного отображения ассоциативной алгебры
   {компонента полилинейного отображения ассоциативной алгебры}%
   {component of polylinear map, associative algebra}%
\Index%195%К%компонента полилинейного отображения тела
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index%196%К%компонента производной Гато второго порядка отображения \Vector f(\Vector x)
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index%633%К%компонента производной Гато второго порядка отображения f(x) алгебры
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Index%197%К%компонента производной Гато второго порядка отображения тела
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index%199%К%компонента производной Гато отображения \Vector f(\Vector x)
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index%198%К%компонента производной Гато отображения f(x)
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index%629%К%компонента производной Гато отображения f(x) алгебры
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%204%К%координатная матрица вектора в rcd базисе
   {координатная матрица вектора в \rcd базисе}%
   {coordinate matrix of vector in rcd basis}%
\Index%691%К%координатная матрица вектора в базисе
   {координатная матрица вектора в базисе}%
   {coordinate matrix of vector in basis, module}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов в векторном пространстве dcr строк
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index%207%К%координатная матрица множества векторов в векторном пространстве rcd строк
   {координатная матрица множества векторов в векторном пространстве \rcd строк}%
   {coordinate matrix of set of vectors, rcd vector space}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора в rcd базисе
   {координаты вектора в \rcd базисе}%
   {coordinates of vector in rcd basis}%
\Index%692%К%координаты вектора в базисе
   {координаты вектора в базисе}%
   {coordinates of vector in basis, module}%
\Index%792%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов в dcr векторном пространстве
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index%223%К%координаты множества векторов в rcd векторном пространстве
   {координаты множества векторов в \rcd векторном пространстве}%
   {coordinates of set of vectors, rcd vector space}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%651%К%косо симметричное полилинейное отображение в ассоциативную алгебру
   {косо симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map skew symmetric, associative algebra}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение тела, порождённое отображением G
   {линейное отображение тела, порождённое отображением $G$}%
   {linear map generated by map, division ring}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%608%Л%линейное отображение  R_1 модуля в R_2 модуль
   {линейное отображение  $R_1$\Hyph модуля $A_1$ в $R_2$\Hyph модуль $A_2$}%
   {linear mapping of R_1 module into R_2 module}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%610%Л%линейное отображение R алгебры в R алгебру
   {линейное отображение $R$\Hyph алгебры $A_1$ в $R$\Hyph алгебру $A_2$}%
   {linear mapping of R algebras}%
\Index%613%Л%линейное отображение R модуля в R модуль
   {линейное отображение $R$\Hyph модуля $A_1$ в $R$\Hyph модуль $A_2$}%
   {linear mapping of R modules}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear mapping of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%801%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {Linear Representation of Lie Group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%803%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%681%М%матрица Acr линейного отображения модуля
   {матрица \Acr линейного отображения модуля}%
   {matrix of Acr linear map}%
\Index%584%М%матрица Astar линейного отображения
   {матрица $A\star$\Hyph линейного отображения}%
   {matrix of Astar linear map}%
\Index%251%М%матрица rcd линейного отображения
   {матрица \rcd линейного отображения}%
   {matrix of rcd linear map}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения D- векторного пространства
   {матрица Якоби\Hyph Гато отображения $D$\Hyph векторного пространства}%
   {Jacobi Gateaux matrix of map, D vector space}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%806%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%813%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor, algebra}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%313%Н%непрерывная функция над алгебро1
   {непрерывная функция над $D$\Hyph алгебро1}%
   {continuous function, algebra}%
\Index%280%Н%непрерывная функция тела
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%346%Н%норма на D- алгебре
   {норма на $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%793%Н%норма на кольце
   {норма на кольце}%
   {absolute value on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%285%Н%норма отображения  тела
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index%286%Н%норма отображения \Vector A нормированного D-векторного пространства
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index%314%Н%норма отображения в D- алгебру
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Index%343%Н%нормированная D- алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%287%Н%нормированное D- векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%794%Н%нормированное кольцо
   {нормированное кольцо}%
   {valued ring}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%802%О%однородное линейное представление группы Ли
   {однородное линейное представление группы Ли}%
   {homogeneous Linear Representation of Lie Group}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%804%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%342%П%полилинейное отображение (n)-D-векторных пространств
   {полилинейное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polylinear map of D vector spaces}%
\Index%609%П%полилинейное отображение алгебр
   {полилинейное отображение алгебр}%
   {polylinear map of algebras}%
\Index%621%П%полилинейное отображение модулей
   {полилинейное отображение модулей}%
   {polylinear map of modules}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%271%П%последовательность Коши в нормированном алгебре
   {последовательность Коши в нормированном алгебрае}%
   {Cauchy sequence, normed algebra}%
\Index%241%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, normed ring}%
\Index%797%П%последовательность Коши в нормированном кольце
   {последовательность Коши в нормированном кольце}%
   {Cauchy sequence, valued ring}%
\Index%351%П%последовательность Коши в нормированном теле
   {последовательность Коши в нормированном теле}%
   {Cauchy sequence, valued division ring}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%460%П%предел последовательности в нормированной алгебре
   {предел последовательности в нормированной алгебре}%
   {limit of sequence, normed algebra}%
\Index%467%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Index%795%П%предел последовательности в нормированном кольце
   {предел последовательности в нормированном кольце}%
   {limit of sequence, valued ring}%
\Index%364%П%предел последовательности в нормированном теле
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка отображения f
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index%626%П%производная Гато второго порядка отображения алгебры
   {производная Гато второго порядка отображения алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Index%397%П%производная Гато отображения f
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index%398%П%производная Гато отображения Vector f нормированого D- векторного пространства Vector V в нормированное D- векторное пространство Vector W
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index%627%П%производная Гато отображения алгебры
   {производная Гато отображения алгебры}%
   {Gateaux derivative of map, algebra}%
\Index%399%П%производная Гато порядка n отображения \Vector f
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index%634%П%производная Гато порядка n отображения f алгебры
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Index%400%П%производная Гато порядка n отображения f тела
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%812%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%781%С%скаляр отображения
   {скаляр отображения}%
   {scalar of mapping}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато отображения f^j по переменным v^i, v^j
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%456%С%стандартная F- компонента линейного отображения f
   {стандартная $F$\Hyph компонента линейного отображения $f$}%
   {standard component of linear map, division ring}%
\Index%458%С%стандартная компонента дифференциала Гато отображения f
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения f тела
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index%630%С%стандартная компонента производной Гато отображения f
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index%574%С%стандартная компонента тензора в тензорном произведении алгебр
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Index%464%С%стандартное F- представление линейного отображения тела
   {стандартное $F$\Hyph представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index%465%С%стандартное представление дифференциала Гато отображения тела над полем F
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%648%С%стандартное представление полилинейного отображения в ассоциативную алгебру
   {стандартное представление полилинейного отображения в ассоциативную алгебру}%
   {polylinear map, standard representation, associative algebra}%
\Index%470%С%стандартное представление полилинейного отображения тела
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index%631%С%стандартное представление производной Гато отображения над алгеброй
   {стандартное представление производной Гато отображения над алгеброй}%
   {Gateaux derivative, standard representation, algebra}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%618%С%структурные константы алгебры над кольцом
   {структурные константы алгебры $P$ над кольцом $D$}%
   {structural constants of algebra}%
\Index%473%С%структурные константы тела D над полем F
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%682%С%сумма Acr линейных отображений модуля
   {сумма \Acr линейных отображений модуля}%
   {sum of Acr linear maps, module}%
\Index%475%С%сумма rcd линейных отображений
   {сумма \rcd линейных отображений}%
   {sum of rcd linear maps, rcd vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%652%Т%тензорная степень алгебры $A$
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Index%763%Т%тензорная степень представления
   {тензорная степень представления}%
   {tensor power of representation}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%762%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%487%Т%топологическое drc векторное пространство
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%808%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%807%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%798%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%796%Ф%фундаментальная последовательность в нормированное кольце
   {фундаментальная последовательность в нормированное кольце}%
   {fundamental sequence, valued ring}%
\Index%500%Ф%фундаментальная последовательность в нормированное теле
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index%243%Ф%фундаментальная последовательность в нормированном алгебре
   {фундаментальная последовательность в нормированном алгебре}%
   {fundamental sequence, normed algebra}%
\Index%642%Ф%фундаментальная последовательность в нормированном кольце
   {фундаментальная последовательность в нормированном кольце}%
   {fundamental sequence, normed ring}%
\Index%502%Ф%функция \gi n D- значных переменных
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index%501%Ф%функция D- векторного пространства V в D- векторное пространство W, дифференцируемая по Гато
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index%625%Ф%функция алгебры, дифференцируемая по Гато
   {функция алгебры, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, algebra}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%505%Ф%функция тела, дифференцируемая по Гато
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index%506%Ф%функция, непрерывная по совокупности аргументов
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\Index%805%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения fb по переменной xa
   {частная \crd производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато отображения f^j по переменной v^i
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index%513%Ч%частное линейное отображение переменной v^i
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения D- векторного пространства
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Index%523%Я%ядро линейного отображения тела
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Linear.Mapping.Russian.tex <==
%auto-ignore
\input{\FilePrefix Linear.Mapping.Eq}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\Chapter{Линейное отображение алгебры}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\Section{Модуль}
\label{Section: Module}

\begin{theorem}
\label{theorem: effective representation of the ring}
Пусть кольцо $D$ имеет единицу $e$.
Представление
\ShowEq{representation of the ring}
кольца $D$
в абелевой группе $A$
\AddIndex{эффективно}{effective representation of ring}
тогда и только тогда, когда
из равенства $f(a)=0$ следует $a=0$.
\end{theorem}
\begin{proof}
Сумма преобразований $f$ и $g$ абелевой группы определяется согласно
правилу
\ShowEq{sum of transformations of Abelian group}
Поэтому, рассматривая представление кольца $D$ в
абелевой группе $A$, мы полагаем
\ShowEq{sum of transformations of Abelian group, 1}
Произведение преобразований представления определено
согласно правилу
\ShowEq{product of transformations of representation}

Если $a$, $b\in R$
порождают одно и то же преобразование, то
\ShowEq{representation of ring, 1}
для любого $m\in A$.
Из равенства
\EqRef{representation of ring, 1}
следует, что $a-b$ порождает нулевое преобразование
\ShowEq{representation of ring, 2}
Элемент $e+a-b$ порождает тождественное преобразование.
Следовательно, представление $f$ эффективно тогда и только тогда,
когда $a=b$.
\end{proof}

\begin{definition}
\label{definition: module over ring}
Пусть $D$ - коммутативное кольцо.
$A$ - \AddIndex{модуль над кольцом}{module over ring} $D$,
если $A$ - абелева группа и
определено эффективное представление кольца $D$
в абелевой группе $A$.
\qed
\end{definition}

\begin{definition}
\label{definition: free module over ring}
Множество векторов
\ShowEq{basis, module}
- \AddIndex{$D\star$\Hyph базис модуля}{D basis, module},
если векторы $\Veb$ $D\star$\Hyph линейно независимы и добавление
любого вектора к этой системе
делает эту систему $D\star$\Hyph линейно зависимой.
$A$ - \AddIndex{свободный модуль над кольцом}{free module over ring} $D$,
если $A$ имеет базис
над кольцом $D$.\footnote{Я следую
определению в \citeBib{Serge Lang}, с. 103.}
\qed
\end{definition}

\begin{theorem}
\label{theorem: free module over ring, change basis}
Пусть $A$ - свободный модуль над кольцом $D$.
Координаты $a^{\gi j}$ вектора $a\in A$
являются координатами $D$-значного контравариантнго тензора
\ShowEq{free module over ring, change basis, 3}
\end{theorem}
\begin{proof}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{free module over ring, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Так как вектор $a$ не меняется, то
\ShowEq{free module over ring, change basis, 1}
Из равенств \EqRef{free module over ring, change basis}
и \EqRef{free module over ring, change basis, 1}
следует
\ShowEq{free module over ring, change basis, 2}
Так как векторы $\Vector e_{\gi j}$ линейно независимы, то равенство
\EqRef{free module over ring, change basis, 3}
следует
из равенства
\EqRef{free module over ring, change basis, 2}.
Следовательно, компоненты вектора являются тензором.
\end{proof}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
Следующее определение является следствием определений
\ref{definition: module over ring}
и \xRef{0912.3315}{definition: morphism of representations of F algebra}.

\begin{definition}
\label{definition: linear map from A1 R1 to A2 R2}
Пусть $A_1$ - модуль над кольцом $R_1$.
Пусть $A_2$ - модуль над кольцом $R_2$.
Морфизм
\ShowEq{linear map from A1 R1 to A2 R2}
представления кольца $R_1$ в абелевой группе $A_1$
в представление кольца $R_2$ в абелевой группе $A_2$
называется
\AddIndex{линейным отображением $R_1$\Hyph модуля $A_1$
в $R_2$\Hyph модуль $A_2$}
{linear mapping of R_1 module into R_2 module}.
\qed
\end{definition}

\begin{theorem}
Линейное отображение
\ShowEq{linear map from A1 R1 to A2 R2}
$R_1$\Hyph модуля $A_1$
в $R_2$\Hyph модуль $A_2$
удовлетворяет равенствам\footnote{Предлагаемые равенства в
классической записи имеют вполне знакомый вид
\ShowEq{linear map from A1 R1 to A2 R2, 1, old}}
\ShowEq{linear map from A1 R1 to A2 R2, 1}
\end{theorem}
\begin{proof}
Из определений
\ref{definition: linear map from A1 R1 to A2 R2}
и \xRef{0912.3315}{definition: morphism of representations of F algebra}
следует, что
\begin{itemize}
\item отображение $f$ является гомоморфизмом кольца $R_1$
в кольцо $R_2$ (равенство
\EqRef{linear map from A1 R1 to A2 R2, 1 3})
\item отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\EqRef{linear map from A1 R1 to A2 R2, 1 1})
\end{itemize}
Равенство
\EqRef{linear map from A1 R1 to A2 R2, 1 2}
следует из равенства
\xEqRef{0912.3315}{morphism of representations of F algebra, definition, 2}.
\end{proof}

Согласно теореме
\xRef{0912.3315}{theorem: morphism of representations of algebra, reduce}
при изучении линейных отображений, не нарушая общности,
мы можем полагать $R_1=R_2$.
\fi

\begin{definition}
\label{definition: linear map from A1 to A2, module}
Пусть $A_1$ и
$A_2$ - модули над кольцом $D$.
Морфизм
\ShowEq{linear map from A1 to A2}
представления кольца $D$ в абелевой группе $A_1$
в представление кольца $D$ в абелевой группе $A_2$
называется
\AddIndex{линейным отображением $D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$}
{linear mapping of R modules}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map from A1 to A2}
Линейное отображение
\ShowEq{linear map from A1 to A2}
$D$\Hyph модуля $A_1$
в $D$\Hyph модуль $A_2$
удовлетворяет равенствам\footnote{В классической записи
приведенные равенства имеют вид
\ShowEq{linear map from A1 to A2, 1 old}
В некоторых книгах
(например, \citeBib{Serge Lang}, с. 94) теорема \ref{theorem: linear map from A1 to A2}
рассматривается как определение.}
\ShowEq{linear map from A1 to A2, 1}
\end{theorem}
\begin{proof}
Из определения
\ref{definition: linear map from A1 to A2, module}
и теоремы
\xRef{0912.3315}{theorem: morphism of representations of algebra, reduce}
следует, что
отображение $g$ является гомоморфизмом абелевой группы $A_1$
в абелеву группу $A_2$ (равенство
\EqRef{linear map from A1 to A2, 1 1})
Равенство
\EqRef{linear map from A1 to A2, 1 2}
следует из равенства
\xEqRef{0912.3315}{morphism of representations of F algebra}.
\end{proof}

\begin{definition}
\label{definition: polylinear map of modules}
Пусть $D$ - коммутативное кольцо.
Пусть $A_1$, ..., $A_n$, $S$ - $D$\Hyph модули.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением модулей}
{polylinear map of modules}
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
\qed
\end{definition}

\Section{Алгебра над кольцом}
\label{section: Algebra over Ring}

\fi%2010.05.23
\else%1011.3102
\section{Алгебра над кольцом}
\fi%1011.3102
\begin{definition}
\label{definition: algebra over ring}
Пусть $D$ - коммутативное кольцо.
\ePrints{1003.1544,8433-5163}
\ifx\Semafor\ValueOn
Пусть $A$ - модуль над кольцом $D$.\footnote{Существует
несколько эквивалентных определений алгебры.
Вначале я хотел рассмотреть представление кольца $D$
в абелевой группе кольца $A$.
Однако мне надо было объяснить почему произведение
элементов кольца $D$ и алгебры $A$ коммутативно.
Это потребовало определение центра алгебры $A$.
После тщательного анализа
я выбрал определение, приведенное в
\citeBib{Richard D. Schafer}, с. 1,
\citeBib{0105.155}, с. 4.
%Эта точка зрения имеет ещё два преимущества.
%Во-первых, как следует из теоремы
%если алгебра не имеет единицы, то не существует
%изоморфного образа кольца $D$ в алгебре $A$.
%Во-вторых, я не исключаю возможность рассматривать
%векторное пространство над алгеброй как алгебру.
}
\else
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Пусть $A$ - модуль над кольцом $D$.\footnote{Этот
подраздел написан на основе раздела
\xRef{8433-5163}{section: Algebra over Ring}.}
\else
Пусть $A$ - модуль над кольцом $D$.
\fi
\fi
Для заданного билинейного отображения
\ShowEq{product in algebra, definition 1}
мы определим произведение в $A$
\ShowEq{product in algebra, definition 2}
$A$ - \AddIndex{алгебра над кольцом}{algebra over ring} $D$,
если $A$ - $D$\Hyph модуль и в $A$
определена операция произведения
\EqRef{product in algebra, definition 2}.
\ePrints{2010.05.23,1011.3102}
\ifx\Semafor\ValueOff
Алгебра
\ShowEq{opposite algebra}
называется
\AddIndex{алгеброй, противоположной алгебре $A$}{opposite algebra},
если в модуле $A$ определено произведение согласно
правилу\footnote{Определение дано по аналогии
с определением \citeBib{Bourbaki: Algebra 1}-2, с. 19.}
\ShowEq{opposite algebra, product}
\fi
Если $A$ является свободным
$D$\Hyph модулем, то $A$ называется
\AddIndex{свободной алгеброй над кольцом}{free algebra over ring} $D$.
\qed
\end{definition}

\ePrints{2010.05.23,1011.3102}
\ifx\Semafor\ValueOff
\begin{remark}
\label{remark: opposite algebra}
Алгебра $A$ и противоположная ей алгебра совпадают как
модули.
\qed
\end{remark}

\begin{theorem}
Произведение в алгебре $A$ дистрибутивно по отношению к сложению.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{product distributive in algebra}
\end{proof}

Произведение в алгебре может быть ни коммутативным,
ни ассоциативным. Следующие определения основаны на
определениях, данным в \citeBib{Richard D. Schafer}, с. 13.

\begin{definition}
\label{definition: commutator of algebra}
\AddIndex{Коммутатор}{commutator of algebra}
\ShowEq{commutator of algebra}
служит мерой коммутативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{коммутативной}{commutative D algebra},
если
\ShowEq{commutative D algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: associator of algebra}
\AddIndex{Ассоциатор}{associator of algebra}
\ShowEq{associator of algebra}
служит мерой ассоциативности в $D$\Hyph алгебре $A$.
$D$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной}{associative D algebra},
если
\ShowEq{associative D algebra}
\qed
\end{definition}

\begin{theorem}
Пусть $A$ - алгебра над коммутативным кольцом $D$.\footnote{Утверждение
теоремы опирается на равенство
\citeBib{Richard D. Schafer}-(2.4).}
\ShowEq{associator of algebra, 1}
для любых $a$, $b$, $c$, $d\in A$.
\end{theorem}
\begin{proof}
Равенство \EqRef{associator of algebra, 1}
следует из цепочки равенств
\ShowEq{associator of algebra, 2}
\end{proof}

\begin{definition}
\label{definition: nucleus of algebra}
\AddIndex{Ядро $D$\Hyph алгебры $A$}{nucleus of algebra}
- это множество\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 13}
\ShowEq{nucleus of algebra}
\qed
\end{definition}

\begin{definition}
\label{definition: center of algebra}
\AddIndex{Центр $D$\Hyph алгебры $A$}{center of algebra}
- это множество\footnote{Определение дано на базе
аналогичного определения в
\citeBib{Richard D. Schafer}, с. 14}
\ShowEq{center of algebra}
\qed
\end{definition}

\begin{theorem}
\label{theorem: unit of algebra and ring}
Пусть $D$ - коммутативное кольцо.
Если $D$\Hyph алгебра $A$ имеет единицу, то существует
изоморфизм $f$ кольца $D$ в центр алгебры $A$.
\end{theorem}
\begin{proof}
Пусть $e\in A$ - единица алгебры $A$.
Положим $f\circ a=ae$.
\end{proof}
\else
\newpage
\fi

Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Если алгебра $A$ имеет единицу,
положим $\Vector e_{\gi 0}$ - единица алгебры $A$.

\begin{theorem}
Пусть $\Basis e$ - базис свободной алгебры $A$ над кольцом $D$.
Пусть
\ShowEq{a b in basis of algebra}
Произведение $a$, $b$ можно получить согласно правилу
\ShowEq{product in algebra}
где
\ShowEq{structural constants of algebra}
- \AddIndex{структурные константы алгебры $A$ над кольцом $D$}
{structural constants of algebra}.
Произведение базисных векторов в алгебре $A$ определено согласно правилу
\ShowEq{product of basis vectors, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Равенство
\EqRef{product of basis vectors, algebra}
является следствием утверждения, что $\Basis e$
является базисом алгебры $A$.
Так как произведение в алгебре является билинейным отображением,
то произведение $a$ и $b$ можно записать в виде
\ShowEq{product in algebra, 1}
Из равенств
\EqRef{product of basis vectors, algebra},
\EqRef{product in algebra, 1},
следует
\ShowEq{product in algebra, 2}
Так как $\Basis e$ является базисом алгебры $A$, то равенство
\EqRef{product in algebra}
следует из равенства
\EqRef{product in algebra, 2}.
\end{proof}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\begin{theorem}
Если алгебра $A$ коммутативна, то
\ShowEq{commutative product in algebra, 1}
Если алгебра $A$ ассоциативна, то
\ShowEq{associative product in algebra, 1}
\end{theorem}
\begin{proof}
Для коммутативной алгебры,
равенство
\EqRef{commutative product in algebra, 1}
следует из равенства
\ShowEq{commutative product in algebra}
Для ассоциативной алгебры,
равенство
\EqRef{associative product in algebra, 1}
следует из равенства
\ShowEq{associative product in algebra}
\end{proof}
\fi
\fi

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Линейное отображение алгебры}
\label{Section: Linear Mapping of Algebra}
\fi

\ePrints{2010.05.23,1011.3102}
\ifx\Semafor\ValueOff
Алгебра является кольцом. Отображение, сохраняющее
структуру алгебры как кольца, называется гомоморфизмом
алгебры. Однако для нас важнее утверждение, что алгебра
является модулем над коммутативным кольцом.
Отображение, сохраняющее
структуру алгебры как модуля, называется линейным отображением
алгебры.
Таким образом,
следующее определение
опирается на определение
\ref{definition: linear map from A1 to A2, module}.
\fi

\begin{definition}
\label{definition: linear map from A1 to A2, algebra}
Пусть $A_1$ и
$A_2$ - алгебры над кольцом $D$.
\ePrints{1011.3102}
\ifx\Semafor\ValueOff
Морфизм
\ShowEq{linear map from A1 to A2}
представления кольца $D$ в абелевой группе $A_1$
в представление кольца $D$ в абелевой группе $A_2$
\else
Линейное отображение\footnote{Этот
подраздел написан на основе раздела
\xRef{8433-5163}{Section: Linear Mapping of Algebra}.}
\ShowEq{linear map from A1 to A2}
$D$\hyph модуля $A_1$
в $D$\hyph модуль $A_2$
\fi
называется
\AddIndex{линейным отображением $D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$}
{linear mapping of R algebras}.
Обозначим
\ShowEq{set linear mappings, algebra}
множество линейных отображений
алгебры
$A_1$
в алгебру
$A_2$.
\qed
\end{definition}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\begin{theorem}
Линейное отображение
\ShowEq{linear map from A1 to A2}
$D$\Hyph алгебры $A_1$
в $D$\Hyph алгебру $A_2$
удовлетворяет равенствам
\ShowEq{linear map from A1 to A2, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: linear map from A1 to A2}.
\end{proof}

\begin{theorem}
\label{theorem: linear map times constant, algebra}
Рассмотрим $D$\Hyph алгебру $A_1$ и $D$\Hyph алгебру $A_2$.
Пусть отображение
\ShowEq{linear map from A1 to A2}
является линейным отображением.
Тогда отображения
\ShowEq{linear map times constant, algebra}
определённые равенствами
\ShowEq{linear map times constant, 0, algebra}
также являются линейными.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{linear map times constant, 1, algebra}
\end{proof}
\fi
\fi

\begin{theorem}
\label{theorem: linear map, 0, D algebra}
Рассмотрим $D$\Hyph алгебру $A_1$ и $D$\Hyph алгебру $A_2$.
Пусть отображение
\ShowEq{linear map from A1 to A2}
является линейным отображением.
Тогда
\ShowEq{linear map, 0, D algebra}
\end{theorem}
\begin{proof}
Следствие равенства
\ShowEq{linear map, 0, D algebra, 1}
\end{proof}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\ePrints{8433-5163,1011.3102}
\ifx\Semafor\ValueOff
\Section{Полилинейное отображение алгебры}
\fi

\begin{definition}
\label{definition: polylinear map of algebras}
Пусть $D$ - коммутативное ассоциативное кольцо.
Пусть $A_1$, ..., $A_n$ -
$D$\Hyph алгебры и $S$ - $D$\Hyph модуль.
Мы будем называть отображение
\ShowEq{polylinear map of algebras}
\AddIndex{полилинейным отображением алгебр}
{polylinear map of algebras}
$A_1$, ..., $A_n$
в модуль $S$,
если
\ShowEq{polylinear map of algebras, 1}
Обозначим
\ShowEq{set polylinear mappings, algebra}
множество полилинейных отображений
алгебр
$A_1$, ..., $A_n$
в модуль
$S$.
Обозначим
\ShowEq{set polylinear mappings An, algebra}
множество $n$\hyph линейных отображений
алгебры $A$ ($A_1=...=A_n=A$)
в модуль
$S$.
\qed
\end{definition}

\ePrints{8433-5163}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: sum of polylinear maps, algebra}
Пусть $D$ - коммутативное ассоциативное кольцо.
Пусть $A_1$, ..., $A_n$ -
$D$\Hyph алгебры и $S$ - $D$\Hyph модуль.
Пусть отображения
\ShowEq{sum of polylinear maps, algebra}
являются полилинейными отображениями.
Тогда отображение $f+g$,
определённое равенством
\ShowEq{sum of polylinear maps, 0, algebra}
также является полилинейным.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{sum of polylinear maps, 1, algebra}
\end{proof}

\begin{corollary}
Рассмотрим алгебру $A_1$ и алгебру $A_2$.
Пусть отображения
\ShowEq{sum of linear maps, algebra}
являются линейными отображениями.
Тогда отображение $f+g$,
определённое равенством
\ShowEq{sum of linear maps, 0, algebra}
также является линейным.
\qed
\end{corollary}

\begin{theorem}
\label{theorem: polylinear map times scalar, algebra}
Пусть $D$ - коммутативное ассоциативное кольцо.
Пусть $A_1$, ..., $A_n$ -
$D$\Hyph алгебры и $S$ - $D$\Hyph модуль.
Пусть отображение
\ShowEq{polylinear map of algebras}
является полилинейным отображением.
Тогда отображение
\ShowEq{linear map times scalar, algebra}
определённое равенством
\ShowEq{linear map times scalar, 0, algebra}
также является полилинейными.
При этом выполняется равенство
\ShowEq{linear map times scalar, pf, algebra}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{polylinear map times scalar, 1, algebra}
\end{proof}

\begin{corollary}
Рассмотрим алгебру $A_1$ и алгебру $A_2$.
Пусть отображение
\ShowEq{linear map from A1 to A2}
является линейным отображением.
Тогда отображение
\ShowEq{linear map times scalar, algebra}
определённое равенством
\ShowEq{linear map times scalar, 0, algebra}
также является линейным.
При этом выполняется равенство
\ShowEq{linear map times scalar, pf, algebra}
\qed
\end{corollary}

\begin{theorem}
\label{theorem: module of polylinear mappings}
Пусть $D$ - коммутативное ассоциативное кольцо.
Пусть $A_1$, ..., $A_n$ -
$D$\Hyph алгебры и $S$ - $D$\Hyph модуль.
Множество \ShowEq{module of polylinear mappings}
является $D$\Hyph модулем.
\end{theorem}
\begin{proof}
Теорема \ref{theorem: sum of polylinear maps, algebra}
определяет сумму полилинейных отображений
в $D$\Hyph модуль $S$.
Пусть
\ShowEq{module of polylinear mappings, 1}
Для любого
\ShowEq{module of polylinear mappings, 2}
Следовательно, сумма полилинейных отображений коммутативна и ассоциативна.

Отображение $z$, определённое равенством
\ShowEq{module of polylinear mappings, 3}
является нулём операции сложения, так как
\ShowEq{module of polylinear mappings, 4}
Для заданного отображения $f$ отображение $g$,
определённое равенством
\ShowEq{module of polylinear mappings, 5}
удовлетворяет равенству
\ShowEq{module of polylinear mappings, 6}
так как
\ShowEq{module of polylinear mappings, 7}
Следовательно, множество $\mathcal L(A_1;A_2)$
является абелевой группой.

Из теоремы
\ref{theorem: polylinear map times scalar, algebra}
следует, что определенно представление
кольца $D$ в абелевой группе $\mathcal L(A_1,...,A_n;S)$.
Так как кольцо $D$ имеет единицу, то
\ePrints{1011.3102}
\ifx\Semafor\ValueOff
согласно теореме
\ref{theorem: effective representation of the ring}
\else
согласно теореме
\xRef{8433-5163}{theorem: effective representation of the ring}
\fi
указанное представление эффективно.
\end{proof}

\begin{corollary}
Пусть $D$ - коммутативное кольцо с единицей.
Рассмотрим $D$\Hyph алгебру $A_1$ и $D$\Hyph алгебру $A_2$.
Множество $\mathcal L(A_1;A_2)$
является $D$\Hyph модулем.
\qed
\end{corollary}
\fi
\fi

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Алгебра \texorpdfstring{$\mathcal L(A;A)$}{L(A;A)}}

\begin{theorem}
\label{theorem: product of linear mapping, algebra}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $B$.
Пусть $g$ - линейное отображение из $D$\Hyph алгебры $B$ в $D$\Hyph алгебру $C$.
Отображение $g\circ f$, определённое диаграммой
\ShowEq{product of linear mapping, algebra}
является линейным отображением из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $C$.
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств
\ShowEq{product of linear mapping, algebra, 1}
\end{proof}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{theorem}
\label{theorem: product of linear mapping, algebra, f}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $f$ - линейное отображение из $D$\Hyph алгебры $A$ в $D$\Hyph алгебру $B$.
Отображение $f$ порождает линейное отображение
\ShowEq{product of linear mapping, algebra, f}
\ShowEq{product of linear mapping, algebra, f diagram}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств\footnote{Мы пользуемся
следующими определениями операций над отображениями
\ShowEq{operations over linear map}
}
\ShowEq{product of linear mapping, algebra, f1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear mapping, algebra, g}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Пусть $g$ - линейное отображение из $D$\Hyph алгебры $B$ в $D$\Hyph алгебру $C$.
Отображение $g$ порождает линейное отображение
\ShowEq{product of linear mapping, algebra, g}
\ShowEq{product of linear mapping, algebra, g diagram}
\end{theorem}
\begin{proof}
Доказательство теоремы следует из цепочек равенств\footnote{Мы пользуемся
следующими определениями операций над отображениями
\ShowEq{operations over linear map}
}
\ShowEq{product of linear mapping, algebra, g1}
\end{proof}
%\fi
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\begin{theorem}
\label{theorem: product of linear mapping, algebra, gf}
Пусть $A$, $B$, $C$ - алгебры над коммутативным кольцом $D$.
Отображение
\ShowEq{product of linear mapping, algebra, gf}
является билинейным отображением.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\else
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: product of linear mapping, algebra, f},
\ref{theorem: product of linear mapping, algebra, g}.
\end{proof}
\fi%2010.05.23
\fi

\begin{theorem}
\label{theorem: module L(A;A) is algebra}
Пусть $A$ - алгебра над коммутативным кольцом $D$.
$D$\Hyph модуль $\mathcal L(A;A)$, оснащённый произведением
\ShowEq{module L(A;A) is algebra}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
\ShowEq{product of linear mapping, algebra 1}
\fi
является алгеброй над $D$.
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOff
Теорема является следствием определения
\ref{definition: algebra over ring}
и теоремы
\ref{theorem: product of linear mapping, algebra, gf}.
\else
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: module L(A;A) is algebra}.
\fi
\end{proof}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

\Input{Tensor.Algebra}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Линейное отображение в ассоциативную алгебру}
\else
\section{Линейное отображение в ассоциативную алгебру}
\fi

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: bilinear mapping A LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения $f\in\mathcal L(A_1;A_2)$
отображение
\ShowEq{bilinear mapping A LA}
является билинейным отображением.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{bilinear mapping A LA, 1}
\end{proof}
\fi

\begin{theorem}
\label{theorem: linear map AA LAA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Для заданного отображения $f\in\mathcal L(A_1;A_2)$
существует линейное отображение
\ShowEq{linear map AA LAA}
определённое равенством
\ShowEq{linear map AA LAA, 1}
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теорем
\xRef{8433-5163}{theorem: bilinear mapping A LA}
и
\xRef{8433-5163}{theorem: linear map AA LAA}.
\else
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear mapping},
\ref{theorem: bilinear mapping A LA}.
\fi
\end{proof}

\begin{theorem}
\label{theorem: algebra A2 representation in LA}
Рассмотрим $D$\Hyph алгебры $A_1$ и $A_2$.
Определим произведение в алгебре $\ATwo$
согласно правилу
\ShowEq{product in algebra AA}
Линейное отображение
\ShowEq{representation A2 in LA}
определённое равенством
\ShowEq{representation A2 in LA, 1}
является представлением\footnote{Определение представления
$\Omega$\Hyph алгебры дано в определении
\xRef{0912.3315}{definition: Tstar representation of algebra}.
}
алгебры $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: algebra A2 representation in LA}
\else
Согласно теореме
\ref{theorem: linear map times constant, algebra},
отображение \EqRef{representation A2 in LA, 1}
является преобразованием модуля $\mathcal L(A_1;A_2)$.
Для данного тензора $c\in \ATwo$
преобразование $h(c)$ является линейным преобразованием
модуля $\mathcal L(A_1;A_2)$, так как
\ShowEq{representation A2 in LA, 2}
Согласно теореме
\ref{theorem: linear map AA LAA},
отображение \EqRef{representation A2 in LA, 1}
является линейным отображением.

Пусть
\ShowEq{algebra A2 representation in LA, 1}
Согласно теореме
\ref{theorem: linear map AA LAA}
\ShowEq{algebra A2 representation in LA, 2}
Следовательно, согласно теореме
\ref{theorem: linear map AA LAA}
\ShowEq{algebra A2 representation in LA, 3}
Поскольку произведение в алгебре $A_2$ ассоциативно, то
\ShowEq{algebra A2 representation in LA, 4}
Следовательно, если мы определим произведение в алгебре $\ATwo$
согласно равенству
\EqRef{product in algebra AA},
то отображение \EqRef{representation A2 in LA}
является морфизмом алгебр.
Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra}
отображение \EqRef{representation A2 in LA, 1}
является представлением алгебры $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.
\fi
\end{proof}

\begin{theorem}
\label{theorem: representation of algebra A2 in LA}
Рассмотрим $D$\Hyph алгебру $A$.
Определим произведение в алгебре $A\otimes A$
согласно правилу
\EqRef{product in algebra AA}.
Представление
\ShowEq{representation AA in LA}
алгебры $A\otimes A$
в модуле $\mathcal L(A;A)$,
определённое равенством
\ShowEq{representation AA in LA, 1}
позволяет отождествить тензор
\ShowEq{product in algebra AA 1}
с отображением
\ShowEq{product in algebra AA 2}, где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: representation of algebra A2 in LA}
\else
Согласно теореме
\ref{theorem: linear map AA LAA},
отображение $f\in\mathcal L(A;A)$ и тензор $d\in A\otimes A$
порождают отображение
\ShowEq{tensor and mapping in A, algebra}
Если мы положим $f=\delta$, $d=a\otimes b$,
то равенство \EqRef{tensor and mapping in A, algebra}
приобретает вид
\ShowEq{tensor and mapping in A, 1, algebra}
Если мы положим
\ShowEq{tensor and mapping in A, 2, algebra}
то сравнение равенств
\EqRef{tensor and mapping in A, 1, algebra} и
\EqRef{tensor and mapping in A, 2, algebra}
даёт основание отождествить действие тензора
$a\otimes b$ с
преобразованием $(a\otimes b)\circ\delta$.
\fi
\end{proof}

Из теоремы \ref{theorem: representation of algebra A2 in LA}
следует, что отображение
\EqRef{representation A2 in LA, 1}
можно рассматривать как произведение отображений
$a\otimes b$ и $f$.
\ePrints{1011.3102}
\ifx\Semafor\ValueOff
Тензор $a\in \ATwo$
\AddIndex{невырожден}{nonsingular tensor, algebra},
если существует
тензор $b\in \ATwo$ такой, что $a\circ b=1\otimes 1$.

\begin{definition}
\begin{sloppypar}
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.\footnote{Определение дано по
аналогии с определением
\xRef{0912.3315}{definition: orbit of Tstar representation of group}.}
\AddIndex{Орбитой линейного отображения}
{orbit of linear mapping}
$f\in\mathcal L(A_1;A_2)$
называется множество
\ShowEq{orbit of linear mapping}
\qed
\end{sloppypar}
\end{definition}
\fi
\fi

\begin{theorem}
\label{theorem: h generated by f, associative algebra}
Рассмотрим $D$\Hyph алгебру $A_1$
и ассоциативную $D$\Hyph алгебру $A_2$.
Рассмотрим представление алгебры $\ATwo$
в модуле $\mathcal L(A_1;A_2)$.
Отображение
\ShowEq{linear map h A1 A2}
порождённое отображением
\ShowEq{linear map f A1 A2}
имеет вид
\ShowEq{h generated by f, associative algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: h generated by f, associative algebra}
\else%
Произвольный тензор $a\in\ATwo$ можно представить в виде
\ShowEq{h generated by f 1, associative algebra}
Согласно теореме \ref{theorem: algebra A2 representation in LA},
отображение \EqRef{representation A2 in LA, 1}
линейно.
Это доказывает утверждение теоремы.
\fi%1011.3102
\end{proof}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\begin{theorem}
\label{theorem: orbit of linear mapping}
Пусть $A_2$ - алгебра с единицей $e$.
Пусть
\ShowEq{orbit of linear mapping, 02}
- невырожденный тензор.
Орбиты линейных отображений
$f\in\mathcal L(A_1;A_2)$
и \ShowEq{orbit of linear mapping, 01}
совпадают
\ShowEq{orbit of linear mapping, f = g}
\end{theorem}
\begin{proof}
Если
\ShowEq{orbit of linear mapping, 1}
то существует
\ShowEq{orbit of linear mapping, 2}
такое, что
\ShowEq{orbit of linear mapping, 3}
Тогда
\ShowEq{orbit of linear mapping, 4}
Следовательно,
\ShowEq{orbit of linear mapping, 5}
\ShowEq{orbit of linear mapping, g in f}

Так как $a$ - невырожденный тензор, то
\ShowEq{orbit of linear mapping, 6}
Если
\ShowEq{orbit of linear mapping, 5}
то существует
\ShowEq{orbit of linear mapping, 2}
такое, что
\ShowEq{orbit of linear mapping, 7}
Из равенств
\EqRef{orbit of linear mapping, 6},
\EqRef{orbit of linear mapping, 7},
следует, что
\ShowEq{orbit of linear mapping, 8}
Следовательно,
\ShowEq{orbit of linear mapping, 1}
\ShowEq{orbit of linear mapping, f in g}

\EqRef{orbit of linear mapping, f = g}
следует из равенств
\EqRef{orbit of linear mapping, g in f},
\EqRef{orbit of linear mapping, f in g}.
\end{proof}

Из теоремы
\ref{theorem: orbit of linear mapping} также следует, что, если
\ShowEq{orbit of linear mapping, 01}
и \ShowEq{orbit of linear mapping, 02}
- вырожденный тензор, то
отношение
\EqRef{orbit of linear mapping, g in f} верно.
Однако основной результат теоремы
\ref{theorem: orbit of linear mapping}
состоит в том, что представления алгебры
$\ATwo$ в модуле $\mathcal L(A_1;A_2)$
порождает отношение эквивалентности в модуле $\mathcal L(A_1;A_2)$.
Если удачно выбрать представители каждого класса эквивалентности,
то полученное множество будет множеством образующих
рассматриваемого представления.\footnote{Множество образующих
представления определено в определении
\xRef{0912.3315}{definition: generating set of representation}.}
\fi
\fi

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Линейное отображение в свободную
конечно мерную ассоциативную алгебру}

\begin{theorem}
Пусть $A_1$ - алгебра
над кольцом $D$.
Пусть $A_2$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis e$ - базис алгебры $A_2$ над кольцом $D$.
Отображение
\ShowEq{standard representation of mapping A1 A2, 1, associative algebra}
порождённое отображением $f\in\mathcal L(A_1;A_2)$
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of mapping A1 A2, 2, associative algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else%2010.05.23
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: standard component of tensor, algebra},
стандартное представление тензора $a$ имеет вид
\ShowEq{standard representation of mapping A1 A2, 3, associative algebra}
Равенство
\EqRef{standard representation of mapping A1 A2, 2, associative algebra}
следует из равенств
\EqRef{standard representation of mapping A1 A2, 1, associative algebra},
\EqRef{standard representation of mapping A1 A2, 3, associative algebra}.
\end{proof}
\fi%2010.05.23

\begin{theorem}
\label{theorem: coordinates of mapping A1 A2, algebra}
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $C_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Координаты отображения
\ShowEq{coordinates of mapping A1 A2, 1}
порождённого отображением $f\in\mathcal(A_1;A_2)$
посредством тензора $a\in\ATwo$, и его стандартные компоненты
связаны равенством
\ShowEq{coordinates of mapping A1 A2, 2, associative algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else%2010.05.23
\end{theorem}
\begin{proof}
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $g$ имеют вид
\ShowEq{coordinates of mappings f g, associative algebra}
Из равенств
\EqRef{coordinates of mapping f, associative algebra},
\EqRef{coordinates of mapping g, associative algebra},
\EqRef{standard representation of mapping A1 A2, 2, associative algebra}
следует
\ShowEq{coordinates of mapping A1 A2, 3, associative algebra}
Так как векторы $\Vector e_{2\cdot\gi k}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
следует из равенства
\EqRef{coordinates of mapping A1 A2, 3, associative algebra}.
\end{proof}

\begin{theorem}
\label{theorem: linear map over ring, matrix}
Пусть $D$ является полем.
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной ассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $C_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Рассмотрим матрицу
\ShowEq{linear map over ring, matrix}
строки которой пронумерованы индексом
\ShowEq{linear map over ring, row of matrix}
и столбцы пронумерованы индексом
\ShowEq{linear map over ring, column of matrix}.
Если
матрица $\mathcal B$ невырождена,
то для заданных координат линейного преобразования
\ShowEq{linear map over ring, left side}
и для отображения
\ShowEq{linear map over ring, f=1},
система линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
относительно стандартных компонент этого преобразования
$g^{\gi{kr}}$ имеет единственное
решение.

Если
матрица $\mathcal B$ вырождена,
то условием существования решения
системы линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
является равенство
\ShowEq{linear map over ring, determinant=0, 1}
В этом случае система линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, associative algebra}
имеет бесконечно много решений и существует линейная
зависимость между величинами $g_{\gi m}^{\gi k}$.
\end{theorem}
\begin{proof}
Утверждение теоремы
является следствием
теории линейных уравнений над полем.
\end{proof}
\fi%2010.05.23

\begin{theorem}
\label{theorem: linear map over ring, determinant=0}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над полем $D$.
Пусть $\Basis e$ - базис алгебры $A$ над полем $D$.
Пусть $C_{\gi{kl}}^{\gi p}$
- структурные константы алгебры $A$.
Пусть матрица \EqRef{linear map over ring, matrix} вырождена.
Пусть линейное отображение $f\in\mathcal L(A;A)$ невырождено.
Если координаты линейных преобразований $f$ и $g$
удовлетворяют равенству
\ShowEq{linear map over ring, determinant=0, 2}
то система линейных уравнений
\ShowEq{coordinates of mapping A}
имеет бесконечно много решений.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else%2010.05.23
\end{theorem}
\begin{proof}
Согласно равенству
\EqRef{linear map over ring, determinant=0, 2}
и теореме
\ref{theorem: linear map over ring, matrix},
система линейных уравнений
\ShowEq{coordinates of mapping A1 A2, 4f}
имеет бесконечно много решений,
соответствующих линейному отображению
\ShowEq{coordinates of mapping A1 A2, 5f}
Согласно равенству
\EqRef{linear map over ring, determinant=0, 2}
и теореме
\ref{theorem: linear map over ring, matrix},
система линейных уравнений
\ShowEq{coordinates of mapping A1 A2, 4g}
имеет бесконечно много решений,
соответствующих линейному отображению
\ShowEq{coordinates of mapping A1 A2, 5g}
Отображения $f$ и $g$ порождены отображением $\delta$.
Согласно теореме
\ref{theorem: orbit of linear mapping},
отображение $f$ порождает отображение $g$.
Это доказывает утверждение теоремы.
\end{proof}
\fi%2010.05.23
\fi%1011.3102

\begin{theorem}
\label{theorem: linear mapping in L(A,A), associative algebra}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над полем $D$.
Представление алгебры $A\otimes A$ в алгебре $\mathcal L(A;A)$ имеет
конечный \AddIndex{базис}{basis of algebra L(A,A)} $\Basis I$.
\begin{enumerate}
\item \label{f in L(A,A), 1, associative algebra}
Линейное отображение
\ShowEq{f in L(A,A)}
имеет вид
\ShowEq{f in L(A,A), 1, associative algebra}
\item \label{f in L(A,A), 2, associative algebra}
Его стандартное представление имеет вид
\ShowEq{f in L(A,A), 2, associative algebra}
\end{enumerate}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else%2010.05.23
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: linear mapping in L(A,A), associative algebra}
\else%1011.3102
Из теоремы \ref{theorem: linear map over ring, determinant=0}
следует, что если матрица $\mathcal B$ вырождена
и отображение $f$ удовлетворяет равенству
\ShowEq{linear map over ring, determinant=0, 3}
то отображение $f$ порождает то же самое множество отображений,
что порождено отображением $\delta$.
Следовательно, для того, чтобы построить базис представления
алгебры $A\otimes A$ в модуле $\mathcal L(A;A)$ мы должны выполнить
следующее построение.

Множество решений системы уравнений
\EqRef{coordinates of mapping A}
порождает свободный подмодуль $\mathcal L$ модуля $\mathcal L(A;A)$.
Мы строим базис $(\Vector h_1, ..., \Vector h_k)$ подмодуля $\mathcal L$.
Затем дополняем этот базис линейно независимыми векторами
$\Vector h_{k+1}$, ..., $\Vector h_m$, которые не принадлежат
подмодулю $\mathcal L$, таким образом, что множество векторов
$\Vector h_1$, ..., $\Vector h_m$
является базисом модуля $\mathcal L(A;A)$.
Множество орбит $(A\otimes A)\circ\delta$,
$(A\otimes A)\circ\Vector h_{k+1}$, ..., $(A\otimes A)\circ\Vector h_m$
порождает модуль $\mathcal L(A;A)$.
Поскольку множество орбит конечно, мы можем выбрать орбиты так, чтобы
они не пересекались. Для каждой орбиты мы можем выбрать
представитель, порождающий эту орбиту.
\fi%1011.3102
\end{proof}
\fi%2010.05.23

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\begin{example}
Для поля комплексных чисел алгебра $\mathcal L(C;C)$ имеет базис
\ShowEq{basis L(C,C)}
Для алгебры кватернионов алгебра $\mathcal L(H;H)$ имеет базис
\ShowEq{basis L(H,H)}
\qed
\end{example}
\fi%1011.3102

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Линейное отображение в неассоциативную алгебру}
\else
\section{Линейное отображение в неассоциативную алгебру}
\fi
\label{Section: Linear Mapping into Nonassociative Algebra}

Так как произведение неассоциативно, мы можем предположить,
что действие $a$, $b\in A$ на отображение $f$ может быть
представленно либо в виде $a(fb)$, либо в виде $(af)b$.
\ePrints{2010.05.23,1011.3102}
\ifx\Semafor\ValueOff
Однако это предположение приводит нас к довольно сложной
структуре линейного отображения.
Чтобы лучше представить насколько сложна структура линейного
отображения, мы начнём с рассмотрения левого и правого сдвигов
в неассоциативной алгебре.

\begin{theorem}
Пусть
\ShowEq{left shift algebra}
отображение левого сдвига.
Тогда
\ShowEq{left shift algebra, 1}
где мы определили линейное отображение
\ShowEq{left shift algebra, 2}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{associator of algebra},
\EqRef{left shift algebra}
следует
\ShowEq{left shift algebra, 3}
Равенство \EqRef{left shift algebra, 1}
следует из равенства \EqRef{left shift algebra, 3}.
\end{proof}
%\ShowEq{left shift algebra, 2a}

\begin{theorem}
Пусть
\ShowEq{right shift algebra}
отображение правого сдвига.
Тогда
\ShowEq{right shift algebra, 1}
где мы определили линейное отображение
\ShowEq{right shift algebra, 2}
\end{theorem}
\begin{proof}
Из равенств
\EqRef{associator of algebra},
\EqRef{right shift algebra}
следует
\ShowEq{right shift algebra, 3}
Равенство \EqRef{right shift algebra, 1}
следует из равенства \EqRef{right shift algebra, 3}.
\end{proof}

Пусть
\ShowEq{f over A}
линейное отображение алгебры $A$.
Согласно теореме \ref{theorem: linear map times constant, algebra},
отображение
\ShowEq{g over A}
также линейное отображение.
Однако неочевидно, можем ли мы записать отображение $g$ в виде
суммы слагаемых вида $(ax)b$ и $a(xb)$.

Если $A$ - свободная конечно мерная алгебра, то мы можем предположить,
что линейное отображение имеет стандартное представление в виде\footnote{Выбор
произволен. Мы можем рассмотреть стандартное представление в виде
\ShowEq{linear map, standard representation, nonassociative algebra, 1}
Тогда равенство
\EqRef{coordinates of mapping A1 A2, 2, nonassociative algebra}
имеет вид
\ShowEq{coordinates of mapping A1 A2, 21, nonassociative algebra}
Я выбрал выражение
\EqRef{linear map, standard representation, nonassociative algebra}
так как порядок сомножителей соответствует порядку, выбранному в теореме
\ref{theorem: linear mapping in L(A,A), associative algebra}.}
\ShowEq{linear map, standard representation, nonassociative algebra}
В этом случае мы можем применить
теорему \ref{theorem: linear mapping in L(A,A), associative algebra}
для отображений в неассоциативную алгебру.
\else%2010.05.23,1011.3102
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi%2010.05.23
\fi%2010.05.23,1011.3102

\begin{theorem}
\label{theorem: coordinates of mapping A1 A2, nonassociative algebra}
Пусть $\Basis e_1$ - базис свободной конечно мерной
$D$\Hyph алгебры $A_1$.
Пусть $\Basis e_2$ - базис свободной конечно мерной неассоциативной
$D$\Hyph алгебры $A_2$.
Пусть $C_{2\cdot}{}_{\gi{kl}}^{\gi p}$ - структурные константы алгебры $A_2$.
Пусть отображение
\ShowEq{standard representation of mapping A1 A2, 1, nonassociative algebra}
порождённое отображением $f\in\mathcal(A_1;A_2)$
посредством тензора $a\in\ATwo$, имеет стандартное представление
\ShowEq{standard representation of mapping A1 A2, 2, nonassociative algebra}
Координаты отображения
\EqRef{standard representation of mapping A1 A2, 1, nonassociative algebra}
и его стандартные компоненты
связаны равенством
\ShowEq{coordinates of mapping A1 A2, 2, nonassociative algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else%2010.05.23
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: coordinates of mapping A1 A2, nonassociative algebra}
\else%1011.3102
Относительно базисов
$\Basis e_1$ и $\Basis e_2$, линейные отображения $f$ и $g$ имеют вид
\ShowEq{coordinates of mappings f g, nonassociative algebra}
Из равенств
\EqRef{coordinates of mapping f, nonassociative algebra},
\EqRef{coordinates of mapping g, nonassociative algebra},
\EqRef{standard representation of mapping A1 A2, 2, nonassociative algebra}
следует
\ShowEq{coordinates of mapping A1 A2, 3, nonassociative algebra}
Так как векторы $\Vector e_{2\cdot\gi k}$
линейно независимы и $x^{\gi i}$ произвольны,
то равенство
\EqRef{coordinates of mapping A1 A2, 2, nonassociative algebra}
следует из равенства
\EqRef{coordinates of mapping A1 A2, 3, nonassociative algebra}.
\fi%1011.3102
\end{proof}
\fi

\begin{theorem}
\label{theorem: linear mapping in L(A,A), nonassociative algebra}
Пусть $A$ - свободная конечно мерная неассоциативная алгебра
над кольцом $D$.
Представление алгебры $A\otimes A$ в алгебре $\mathcal L(A;A)$ имеет
конечный базис $\Basis I$.
\begin{enumerate}
\item \label{f in L(A,A), 1, nonassociative algebra}
Линейное отображение
\ShowEq{f in L(A,A)}
имеет вид
\ShowEq{f in L(A,A), 1, nonassociative algebra}
\item \label{f in L(A,A), 2, nonassociative algebra}
Его стандартное представление имеет вид
\ShowEq{f in L(A,A), 2, nonassociative algebra}
\end{enumerate}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else%2010.05.23
\end{theorem}
\begin{proof}
\ePrints{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: linear mapping in L(A,A), nonassociative algebra}
\else%1011.3102
Рассмотрим матрицу
\EqRef{linear map over ring, matrix}.
Если
матрица $\mathcal B$ невырождена,
то для заданных координат линейного преобразования
\ShowEq{linear map over ring, left side}
и для отображения
\ShowEq{linear map over ring, f=1},
система линейных уравнений
\EqRef{coordinates of mapping A1 A2, 2, nonassociative algebra}
относительно стандартных компонент этого преобразования
$g^{\gi{kr}}$ имеет единственное
решение.
Если
матрица $\mathcal B$ вырождена,
то согласно теореме
\ref{theorem: linear mapping in L(A,A), associative algebra}
существует конечный базис $\Basis I$,
порождающий множество линейных отображений.
\fi%1011.3102
\end{proof}
\fi%2010.05.23

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
В отличие от случая ассоциативной алгебры
множество генераторов $I$ в теореме
\ref{theorem: linear mapping in L(A,A), nonassociative algebra}
не является минимальным.
Из равенства \EqRef{left shift algebra, 1}
следует, что неверно равенство
\EqRef{orbit of linear mapping, 4}.
Следовательно, орбиты отображений
$I_k$ не порождают отношения эквивалентности в алгебре $L(A;A)$.
Так как мы рассматриваем только отображения вида $(aI_k)b$, то
возможно, что при $k\ne l$ отображение $I_k$ порождает отображение $I_l$,
если рассмотреть все возможные операции в алгебре $A$.
Поэтому множество образующих $I_k$ неассоциативной алгебры $A$
не играет такой критической роли как отображение сопряжения в
поле комплексных чисел.
Ответ на вопрос насколько важно отображение $I_k$ в
неассоциативной алгебре требует дополнительного исследования.
\else%1011.3102

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Полилинейное отображение в ассоциативную алгебру}
\else
\section{Полилинейное отображение в ассоциативную алгебру}
\fi

\begin{theorem}
\label{theorem: polylinear mapping A 1n A}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Пусть
\ShowEq{set of mappings, L(A;A)}
\ShowEq{set of elements A}
Для заданной перестановки $\sigma$ $n$ переменных
отображение
\ShowEq{n linear mapping A LA}
является $n$\hyph линейным отображением в алгебру $A$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{polylinear mapping A 1n A, 1}
\end{proof}

В равенстве \EqRef{n linear mapping A LA},
также как и в других выражениях полилинейного отображения,
принято соглашение, что отображение $f_i$ имеет своим аргументом переменную $x_i$.

\begin{theorem}
\label{theorem: polylinear mapping A LA}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного семейства отображений
\ShowEq{set of mappings, L(A;A)}
отображение
\ShowEq{n+1 linear mapping A LA}
определённое равенством
\ShowEq{n+1 linear mapping A LA 1}
является $n+1$\hyph линейным отображением в $D$\Hyph модуль $\LAAnA$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{n+1 linear mapping A LA, 1}
\end{proof}

\begin{theorem}
\label{theorem: linear map An LAAnA}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного семейства отображений
\ShowEq{set of mappings, L(A;A)}
существует линейное отображение
\ShowEq{linear map An LAAnA}
определённое равенством
\ShowEq{linear map An LAAnA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear mapping},
\ref{theorem: polylinear mapping A LA}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear mapping A LA, 1}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного тензора
\ShowEq{tensor over A} и заданной перестановки $\sigma\in S_n$
отображение
\ShowEq{n linear mapping LA LA}
определённое равенством
\ShowEq{n linear mapping LA LA 1}
является $n$\hyph линейным отображением в $D$\Hyph модуль $\LAAnA$.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочек равенств
\ShowEq{representation An in LAAnA, 3}
\end{proof}

\begin{theorem}
\label{theorem: linear mapping LA LA, 1}
Пусть $A_1$, ..., $A_n$, $A$ - ассоциативные $D$\Hyph алгебры.
Для заданного тензора
\ShowEq{tensor over A} и заданной перестановки $\sigma\in S_n$
существует линейное отображение
\ShowEq{linear mapping LA LA}
определённое равенством
\ShowEq{linear mapping LA LA, 1}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теорем
\ref{theorem: tensor product and polylinear mapping},
\ref{theorem: polylinear mapping A LA, 1}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map, algebra}
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Полилинейное отображение
\ShowEq{polylinear map, algebra}
имеет вид
\ShowEq{polylinear map, algebra, canonical morphism}
где $\sigma_s$ - перестановка множества переменных
\ShowEq{transposition of set of variables, algebra}
\end{theorem}
\begin{proof}
Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является следствием
утверждения \eqref{f in L(A,A), 1, associative algebra} теоремы
\ref{theorem: linear mapping in L(A,A), associative algebra}.
При этом мы можем отождествить\footnote{В представлении
\EqRef{polylinear map, algebra, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}}
\ShowEq{polylinear map, associative algebra, 1, canonical morphism}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\EqRef{polylinear map, algebra}
можно представить в виде
\ShowEq{polylinear map, induction on n, 1, associative algebra}
Согласно предположению индукции полилинейное отображение
$h$ имеет вид
\ShowEq{polylinear map, induction on n, 2, associative algebra}
Согласно построению $h=g\circ a_k$.
Следовательно, выражения $h_{t\cdot p}$
являются функциями $a_k$.
Поскольку $g\circ a_k$ - линейная функция $a_k$,
то только одно выражение $h_{t\cdot p}$
является линейной функцией переменной $a_k$, и остальные выражения
$h_{t\cdot q}$
не зависят от $a_k$.

Не нарушая общности, положим $p=0$.
Согласно равенству
\EqRef{h generated by f, associative algebra}
для заданного $t$
\ShowEq{polylinear map, induction on n, 3, associative algebra}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, induction on n, 4, associative algebra}
Положим
\ShowEq{polylinear map, induction on n, 5, associative algebra}
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\ShowEq{component of polylinear map, associative algebra}
в равенстве \EqRef{polylinear map, algebra, canonical morphism}
называется \AddIndex{компонентой полилинейного отображения $f$}
{component of polylinear map, associative algebra}.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: representation module An in LAAnA}
Рассмотрим $D$\Hyph алгебру $A$.
\ifx\texFuture\Defined
Определим произведение в алгебре $\AOn$
согласно правилу
\ShowEq{product in algebra An}
\fi
Линейное отображение
\ShowEq{representation An in LAnA}
определённое равенством
\ShowEq{representation An in LAnA, 1}
является представлением\footnote{Определение представления
$\Omega$\Hyph алгебры дано в определении
\xRef{0912.3315}{definition: Tstar representation of algebra}.}
алгебры
\ShowEq{representation An in LAnA, 2}
в $D$\Hyph модуле $\LAnA$.
\end{theorem}
\begin{proof}
Согласно теоремам
\ref{theorem: linear mapping in L(A,A), associative algebra},
\ref{theorem: polylinear map, algebra},
$n$\hyph линейное отображение можно представить в виде суммы слагаемых
\EqRef{n linear mapping A LA},
где $f_i$, $i=1$, ..., $n$, генераторы представления
\EqRef{representation A2 in LA}.
Запишем слагаемое $s$ выражения
\EqRef{polylinear map, algebra, canonical morphism}
в виде
\ShowEq{n linear mapping A LA, 1}
где
\ShowEq{n linear mapping A LA, 2}
Положим в равенстве
\EqRef{n linear mapping A LA, 1}
\ShowEq{n linear mapping A LA, 3}
Следовательно, согласно теореме
\ref{theorem: linear map An LAAnA},
отображение \EqRef{representation An in LAnA, 1}
является преобразованием модуля $\LAnA$.
Для данного тензора $c\in \AOn$
и заданной перестановки $\sigma\in S_n$,
преобразование $h(c,\sigma)$ является линейным преобразованием
модуля $\LAnA$
согласно теореме \ref{theorem: linear mapping LA LA, 1}.
Согласно теореме
\ref{theorem: linear map An LAAnA},
отображение \EqRef{representation An in LAnA, 1}
является линейным отображением.
\ifx\texFuture\Defined
Пусть
\ShowEq{algebra An representation in LAnA, 1}
Согласно теореме
\ref{theorem: linear mapping LA LA, 1}
\ShowEq{algebra An representation in LAnA, 2}
Следовательно, согласно теореме
\ref{theorem: linear mapping LA LA, 1}
\ShowEq{algebra An representation in LAnA, 3}
Поскольку произведение в алгебре $A$ ассоциативно, то
\ShowEq{algebra An representation in LAnA, 4}
Следовательно, если мы определим произведение в алгебре $\AOn$
согласно равенству
\EqRef{product in algebra An},
то отображение \EqRef{representation An in LAnA, 1}
является морфизмом алгебр.
\fi
Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra}
отображение \EqRef{representation An in LAnA, 1}
является представлением алгебры
\ShowEq{representation An in LAnA, 2}
в модуле $\LAnA$.
\end{proof}

\begin{theorem}
\label{theorem: representation of algebra An in LAnA}
Рассмотрим $D$\Hyph алгебру $A$.
Представление
\ShowEq{representation An in LAnA}
алгебры $\AOn$
в модуле $\LAnA$,
определённое равенством
\EqRef{representation An in LAnA, 1}
позволяет отождествить тензор
\ShowEq{product in algebra An 1}
и перестановку $\sigma\in S^n$
с отображением
\ShowEq{product in algebra An 2} где
\ShowEq{product in algebra AA 3}
- тождественное отображение.
\end{theorem}
\begin{proof}
Если в равенстве \EqRef{linear map An LAAnA, 1}
мы положим $f_i=\delta$,
\ShowEq{n tensor and mapping in A, 3, algebra},
то равенство \EqRef{linear map An LAAnA, 1}
приобретает вид
\ShowEq{n tensor and mapping in A, 1, algebra}
Если мы положим
\ShowEq{n tensor and mapping in A, 2, algebra}
то сравнение равенств
\EqRef{n tensor and mapping in A, 1, algebra} и
\EqRef{n tensor and mapping in A, 2, algebra}
даёт основание отождествить действие тензора
\ShowEq{n tensor and mapping in A, 3, algebra}
и перестановки $\sigma\in S^n$
с отображением \EqRef{product in algebra An 2}.
\end{proof}

Вместо записи $(a_0\otimes...a_n,\sigma)$ мы также будем пользоваться
записью
\[
a_0\otimes_{\sigma(1)}...\otimes_{\sigma(n)}a_n
\]
если мы хотим явно указать какой аргумент становится на соответствующее место.
Например, следующие выражения эквивалентны
\ShowEq{example of tensor notation}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Полилинейное отображение в свободную
конечно мерную ассоциативную алгебру}
\else
\section{Полилинейное отображение в свободную
конечно мерную ассоциативную алгебру}
\fi

\begin{theorem}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis I$ - базис алгебры $\mathcal L(A;A)$.
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
\AddIndex{Стандартное представление полилинейного отображения в ассоциативную алгебру}
{polylinear map, standard representation, associative algebra}
имеет вид
\ShowEq{polylinear map, associative algebra, standard representation}
Индекс $t$ нумерует всевозможные перестановки
$\sigma_t$ множества переменных
\VarSet.
Выражение
$\ShowSymbol{standard component of polylinear map, associative algebra}$
в равенстве \EqRef{polylinear map, associative algebra, standard representation}
называется \AddIndex{стандартной компонентой полилинейного отображения $f$}
{standard component of polylinear map, division ring}.
\end{theorem}
\begin{proof}
Мы изменим индекс $s$ в равенстве
\EqRef{polylinear map, algebra, canonical morphism}
таким образом, чтобы сгруппировать слагаемые с одинаковым набором генераторов $I_k$.
Выражение \EqRef{polylinear map, algebra, canonical morphism}
примет вид
\ShowEq{polylinear map, algebra, canonical morphism, 1}
Мы предполагаем, что индекс $s$ принимает значения, зависящие от $k_1$, ..., $k_n$.
Компоненты полилинейного отображения $f$
имеют разложение
\ShowEq{polylinear map, associative algebra, components extention}
относительно базиса $\Basis e$.
Если мы подставим \EqRef{polylinear map, associative algebra, components extention}
в \EqRef{polylinear map, algebra, canonical morphism},
мы получим
\ShowEq{polylinear map, associative algebra, standard representation, 1}
Рассмотрим выражение
\ShowEq{polylinear map, associative algebra, standard representation, 2}
В правой части подразумевается сумма тех слагаемых с индексом $s$,
для которых перестановка $\sigma_s$ совпадает. Каждая такая сумма
будет иметь уникальный индекс $t$.
Подставив в равенство
\EqRef{polylinear map, associative algebra, standard representation, 1}
выражение
\EqRef{polylinear map, associative algebra, standard representation, 2}
мы получим равенство \EqRef{polylinear map, associative algebra, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map over field, associative algebra}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
Полилинейное отображение
\EqRef{polylinear map, algebra}
можно представить в виде $D$-значной формы степени $n$
над кольцом $D$\footnote{Теорема доказана по аналогии
с теоремой в \citeBib{Rashevsky}, с. 107, 108}
\ShowEq{polylinear map over ring, associative algebra}
где
\ShowEq{polylinear map over ring, coordinates, associative algebra}
и величины $f_{\gi{i_1...i_n}}$
являются координатами $D$-значного ковариантнго тензора.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: polylinear map of algebras}
равенство
\EqRef{polylinear map over ring, associative algebra}
следует из цепочки равенств
\ShowEq{polylinear map over ring, 1, associative algebra}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{polylinear map over ring, associative algebra, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Из равенств \EqRef{polylinear map over ring, associative algebra, change basis}
и \EqRef{polylinear map over ring, coordinates, associative algebra}
следует
\ShowEq{polylinear map over ring, associative algebra, change coordinates}
Из равенства \EqRef{polylinear map over ring, associative algebra, change coordinates}
следует тензорный закон преобразования координат полилинейного отображения.
Из равенства \EqRef{polylinear map over ring, associative algebra, change coordinates}
и теоремы
\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\ref{theorem: free module over ring, change basis}
\else
\xRef{8433-5163}{theorem: free module over ring, change basis}
\fi
следует, что значение отображения $f\circ(\Vector a_1,...,\Vector a_n)$ не зависит от выбора
базиса.
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, algebra}
\AddIndex{симметрично}
{polylinear map symmetric, associative algebra}, если
\ShowEq{polylinear map symmetric, associative algebra, definition}
для любой перестановки $\sigma$ множества \VarSet.

\begin{theorem}
\label{theorem: polylinear map symmetric, associative algebra}
Если полилинейное отображение $f$ симметрично,
то
\ShowEq{polylinear map symmetric, associative algebra}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map symmetric, associative algebra}
следует из равенства
\ShowEq{polylinear map symmetric, 1, associative algebra}
\end{proof}

Полилинейное отображение
\EqRef{polylinear map, algebra}
\AddIndex{косо симметрично}
{polylinear map skew symmetric, associative algebra}, если
\ShowEq{polylinear map skew symmetric, associative algebra, definition}
для любой перестановки $\sigma$ множества \VarSet.
Здесь
\[
|\sigma|=
\left\{
\begin{matrix}
1&\textrm{перестановка }\sigma\textrm{ чётная}
\\
-1&\textrm{перестановка }\sigma\textrm{ нечётная}
\end{matrix}
\right.
\]

\begin{theorem}
\label{theorem: polylinear map skew symmetric, associative algebra}
Если полилинейное отображение $f$ косо симметрично,
то
\ShowEq{polylinear map skew symmetric, associative algebra}
\end{theorem}
\begin{proof}
Равенство
\EqRef{polylinear map skew symmetric, associative algebra}
следует из равенства
\ShowEq{polylinear map skew symmetric, 1, associative algebra}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of polylinear map, associative algebra over ring}
Пусть $A$ - свободная конечно мерная ассоциативная алгебра
над кольцом $D$.
Пусть $\Basis I$ - базис алгебры $\mathcal L(A;A)$.
Пусть $\Basis e$ - базис алгебры $A$ над кольцом $D$.
Пусть полилинейное над кольцом $D$ отображение $f$
порождено набором отображений $(I_{k_1},...,I_{k_n})$.
Координаты отображения $f$
и его компоненты относительно базиса $\Basis e$
удовлетворяют равенству
\ShowEq{coordinates of polylinear map, associative algebra over ring}
\end{theorem}
\begin{proof}
В равенстве \EqRef{polylinear map, associative algebra, standard representation}
положим
\ShowEq{coordinates of polylinear map, 1, associative algebra over ring}
Тогда равенство \EqRef{polylinear map, associative algebra, standard representation}
примет вид
\ShowEq{polylinear map, associative algebra, standard representation, 1a}
Из равенства \EqRef{polylinear map over ring, associative algebra}
следует
\ShowEq{polylinear map over field, associative algebra, 1a}
Равенство
\EqRef{coordinates of polylinear map, associative algebra over ring}
следует из сравнения равенств
\EqRef{polylinear map, associative algebra, standard representation, 1a}
и
\EqRef{polylinear map over ring, associative algebra}.
Равенство
\EqRef{coordinates of polylinear map, associative algebra over ring, 1}
следует из сравнения равенств
\EqRef{polylinear map, associative algebra, standard representation, 1a}
и
\EqRef{polylinear map over field, associative algebra, 1a}.
\end{proof}
\fi%1011.3102


==> Preface.1006.2597.Russian.tex <==
%auto-ignore
\input{Preface.1006.2597.Eq}

%\chapter{Предисловие}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\section{Предисловие}

В основе математического
анализа лежит возможность линейного приближения к отображению,
и основные построения математического анализа уходят корнями в линейную
алгебру.
Следовательно, прежде чем давать определение
дифференцируемой функции мы должны понять как выглядят
отображения, с помощьью которых мы хотим аппроксимировать
поведение исходной функции.

Так как произведение в поле
коммутативно, то линейная алгебра над полем относительно проста.
При переходе к телу, где произведение некоммутативно, некоторые утверждения линейной
алгебры сохраняются, но появляются и новые утверждения, которые
меняют ландшафт линейной алгебры.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi

Здесь я хочу обратить внимание на эволюцию,
которую претерпело понятие производной со времён Ньютона.
Когда мы изучаем функции одной переменной, то производная в заданной точке
является числом.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\ShowEq{derivative single variable}
\fi
Когда мы изучаем функцию нескольких переменных, выясняется,
что числа недостаточно. Производная становится вектором или градиентом.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\ShowEq{derivative multiple variables}
\newpage
\fi
При изучении отображений векторных пространств мы впервые говорим о производной
как об операторе.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\ShowEq{derivative vector variables}
\fi
Но так как этот оператор линеен, то мы можем представить
производную как матрицу.
И в этом случае мы можем представить вектор приращения функции
как произведение матрицы производной (матрицы Якоби) на
вектор приращения аргумента.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\ShowEq{derivative vector variables 1}
\newpage
\else

Без сомнения, подобное поведение производной ослабляет наше внимание.
Когда мы переходим к объектам, более сложным чем поля или векторные пространства,
мы по прежнему пытаемся увидеть объект, который можно записать как множитель
перед приращением и который от приращения не зависит.
\fi

Предположение, что производная отображения $f$
над алгеброй $A$ определена равенством
\ShowEq{Frechet derivative, algebra}
вначале выглядит привлекательным.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
Однако, положим $f(x)=f_1(x)f_2(x)$. Согласно равенству
\EqRef{Frechet derivative, algebra},\footnote{В последнем звене равенства
\EqRef{Frechet derivative, algebra 1},
мы воспользовались утверждением
\ShowEq{Frechet derivative, algebra 2}
}
\ShowEq{Frechet derivative, algebra 1}
Из равенства
\EqRef{Frechet derivative, algebra},
также следует
\ShowEq{Frechet derivative, algebra 3}
Из равенств
\EqRef{Frechet derivative, algebra 1}
и
\EqRef{Frechet derivative, algebra 3}
следует
\ShowEq{Frechet derivative, algebra 4}
Мы не можем избавиться от величины $h$ в равенстве
\EqRef{Frechet derivative, algebra 4}.
Следовательно,
\else
На первый взгляд подобное определение удовлетворяет
классическим свойствам производной отображения над полем.
Однако
\fi
произведение дифференцируемых функций,
вообще говоря, не является дифференцируемой функцией.
Это приводит к тому, что множество дифференцируемых функций
крайне бедно, а сама теория дифференцирования не представляет
серьёзного интереса.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
Существует ли более широкий класс отображений, который мог бы
содержать производные различных функций?
Чтобы ответить на этот вопрос, рассмотрим отображение $y=x^2$
\ShowEq{mapping y=x2}
Отображение
\ShowEq{mapping y=x2 1}
не является линейным отображением над алгеброй $A$,
но является линейным отображением над центром алгебры $A$.
\else
Поскольку алгебра является модулем над некоторым коммутативным
кольцом существует два пути изучения структур, порождённых
над алгеброй.\footnote{Для изучения
операции дифференцирования в алгебре существует ещё один
метод изучения. Выделив некоторое множество функций,
мы можем определить дифференциальные операторы,
действующие на этом множестве (\citeBib{Serge Lang}, с. 301).

Например, в статье \citeBib{math.CV-0405471}
Людковский рассматривает дифференциальные операторы $\Pza$ и $\Pzb$
в алгебре Кэли - Диксона такие, что
\ShowEq{Ludkovsky differential operators}
Рассматривая заданные свойства дифференциального оператора,
Людковский изучает его структуру.

Изучение оператора дифференцирования с разных точек зрения
даст более глубокое знание и я полагаю в будущем рассмотреть
связь между разными подходами к теории дифференцирования.
}

Если алгебра является свободным модулем, то мы можем выбрать
базис и рассматривать все операции в координатах относительно
заданного базиса.
Хотя базис может быть произвольным, мы можем выбрать наиболее простой
базис с точки зрения алгебраических операций.
Этот подход имеет без сомнения то преимущество,
что мы работаем в коммутативном кольце, где все операции
хорошо изучены.

Рассмотрение операции в алгебре независимо
от выбранного базиса даёт возможность рассматривать элементы
алгебры как самостоятельные объекты.
Однако некоммутативность произведения в алгебре порождает немало
трудностей на этом пути.

Если определение производной \EqRef{Frechet derivative, algebra}
ограничивает нашу возможность изучения поведения
отображений в малом, существует ли альтернатива?
Ответ на этот вопрос положительный.
Мы изучаем математический анализ в алгебре,
которая является нормированым модулем.
Мы знаем два типа производных в нормированном пространстве.
Сильная производная или
производная Фреше является аналогом производной
\EqRef{Frechet derivative, algebra}.
Помимо сильной производной существует слабая производная или производная Гато.
Основная идея состоит в том, что дифференциал может зависеть от направления.

Алгебра $A$ является
модулем над коммутативным кольцом $D$. Если мы ослабим определение
производной и потребуем, что производная отображения $f$ является линейным
отображением модуля $A$, то мы увидим, что по крайней мере
полиномы в алгебре $A$ являются дифференцируемыми отображениями.
Определённая таким образом производная обладает многими свойствами
производной отображений над полем.
\fi
Следовательно, в алгебре из-за некоммутативности умножения
дифференциал
функции имеет слагаемые вида
\ShowEq{adxb}
и мы не можем записать дифференциал отображения
в виде произведения производной и дифференциала аргумента.

Гамильтон был первым, кто рассмотрел
дифференциал отображения в алгебре кватернионов
(\citeBib{Hamilton Elements of Quaternions 1}).
Повидимому, его результаты
были настолько необычны, что
для его современников было трудно воспринять
эту идею Гамильтона и последующие поколения забыли это
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
исследование.
\else
исследование.\footnote{В статье
\citeBib{W.Bertram H.Glockner K.Neeb}
рассмотренна производная Гато отображений модулей над
коммутативным кольцом.
Так как произведение коммутативно, то утверждения в
статье близки к утверждениям классического математического анализа.
Производная определена как отображение дифференциала аргумента
в дифференциал функции.}
\fi

Проблема невозможности разделить
производную и дифференциал настолько серьёзна, что когда Гато определил
слабое дифференцирование, он рассматривал производную только
в том случае, когда он мог выделить приращение аргумента как сомножитель.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
Однако, насколько серьёзно это препятствие?
Производная - это отображение дифференциала аргумента
в дифференциал функции.
Другими словами, производная - это некоторый алгоритм,
на вход которого мы вводим дифференциал аргумента, а
на выходе мы получаем дифференциал функции.
Если мы рассмотрим функциональную запись для линейного отображения, а именно
\ShowEq{functional notation for linear mapping}
то мы можем формально выделить из производной дифференциал аргумента
и сделать запись дифференциала функции
\ShowEq{Gateaux differential}
более знакомой, а именно
\ShowEq{Gateaux differential, 1}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
Тензорное произведение алгебр позволяет явно записать
структуру производной как оператора.

Кроме того, новая запись позволила упростить многие выражения.
Например, выражение
\ShowEq{differential vector function}
приобретает форму
\ShowEq{differential vector function, 1}

Также как и в случае отображений над полем, дифференциал
отображения над алгеброй является многочленом первой степени
относительно приращения аргумента.
Структура полинома над телом отличается от структуры полинома над полем.
Я рассматриваю некоторые свойства полинома в разделе
\ref{section: Taylor Series}.
Опираясь на полученные результаты, я изучаю разложение
отображения в ряд Тейлора и метод
решения дифференциального уравнения.
\fi



==> Second.Derivative.Russian.tex <==
%auto-ignore

\input{\FilePrefix Second.Derivative.Eq}

\Chapter{Производная второго порядка отображения тела}
\label{chapter: Derivative of Second Order of Map of Division Ring}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
{\bf Производная второго порядка отображения алгебры}
\fi
\Section{Производная второго порядка отображения алгебры}

Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Пусть
\ShowEq{f:A->A}
функция, дифференцируемая по Гато.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
Согласно замечанию \ref{remark: differential L(A,A)}
производная Гато является отображением
\ShowEq{differential L(A,A), 2}
Согласно теореме
\ShowEq{theorem: module L(A;A) is algebra}
и определению \ref{definition: norm of map, algebra}
множество $\LAA$ является
банаховой $D$\Hyph алгеброй.
Следовательно, мы можем рассмотреть вопрос,
является ли отображение $\partial f$ дифференцируемым по Гато.

Согласно определению
\ref{definition: function differentiable in Gateaux sense, algebra}
\ShowEq{Gateaux differential of map df, algebra}
где
\ShowEq{Gateaux differential of map df, algebra, o2}
- такое непрерывное отображение, что
\ShowEq{Gateaux differential of map df, algebra, o2 lim}
Согласно определению
\ref{definition: function differentiable in Gateaux sense, algebra}
отображение
\ShowEq{increment of derivative, algebra}
линейно по переменной $a_2$. Из равенства
\EqRef{Gateaux differential of map df, algebra}
следует, что отображение
\ShowEq{increment of derivative, algebra}
линейно по переменной $a_1$.
Следовательно, отображение
\ShowEq{increment of derivative, algebra}
билинейно.
\fi

\begin{definition}
\label{definition: Gateaux derivative of Second Order, algebra}
Полилинейное отображение
\ShowEq{Gateaux derivative of Second Order, algebra}
называется
\AddIndex{производной Гато второго порядка отображения $f$}
{Gateaux derivative of Second Order, algebra}.
\qed
\end{definition}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{remark}
Согласно определению
\ref{definition: Gateaux derivative of Second Order, algebra}
при заданном $x$ производная Гато второго порядка
\ShowEq{differential L(A,A;A), 1}.
Следовательно, производная Гато второго порядка отображения $f$
является отображением
\ShowEq{differential L(A,A;A)}
Согласно теореме
\ShowEq{theorem: tensor product and polylinear mapping}
мы можем также рассматривать отображение
\ShowEq{differential AA A,A}
Тогда
\ShowEq{differential L(AA;A)}
Мы будем пользоваться тем же символом для обозначения отображения,
так как по характеру аргумента ясно о каком отображении идёт речь.
\qed
\end{remark}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{theorem}
Мы можем представить
\AddIndex{дифференциал Гато второго порядка отображения $f$}
{Gateaux differential of Second Order, algebra}
в виде
\ShowEq{Differential of Second Order, algebra, representation}
Мы будем называть выражение
\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\footnote{Мы полагаем
\ShowEq{component of Gateaux derivative of Second Order, 1, algebra}
}
\fi
\ShowEq{component of Gateaux derivative of Second Order, algebra}
\AddIndex{компонентой производной Гато второго порядка отображения $f(x)$}
{component of Gateaux derivative of Second Order, algebra}.
\ePrints{2010.05.23,1006.2597}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\else
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: Gateaux derivative of Second Order, algebra}
и теоремы
\ref{theorem: polylinear map, algebra}.
\end{proof}
\fi

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
По индукции, предполагая, что определена производная Гато
$\partial^{n-1} f(x)$ порядка $n-1$, мы определим
\ShowEq{Gateaux derivative of Order n, algebra}
\AddIndex{производную Гато порядка $n$ отображения $f$}
{Gateaux derivative of Order n, algebra}.
Мы будем также полагать $\partial^0 f(x)=f(x)$.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
{\bf Ряд Тейлора}
\fi
\Section{Ряд Тейлора}
\label{section: Taylor Series}

Пусть $D$ - полное коммутативное кольцо характеристики $0$.
Пусть $A$ - ассоциативная $D$\Hyph алгебра.
Пусть $p_k(x)$ - одночлен степени $k$, $k>0$,
одной переменной над $D$\Hyph алгеброй $A$.

Очевидно, что одночлен степени $0$ имеет вид $a_0$, $a_0\in A$.
Для $k>0$,
\[
p_k(x)=p_{k-1}(x)xa_k
\]
где $a_k\in A$.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
Действительно, последний множитель одночлена $p_k(x)$ является либо $a_k\in A$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.

\fi
В частности, одночлен степени $1$ имеет вид $p_1(x)=a_0xa_1$.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
Не нарушая общности, мы можем положить $k=n$.

\begin{theorem}
\label{theorem: Gateaux derivative of f(x)x, algebra}
Для произвольного $m>0$ справедливо равенство
\ShowEq{Gateaux derivative of f(x)x, algebra}
где символ $\widehat{h^i}$ означает отсутствие переменной $h^i$ в списке.
\end{theorem}
\begin{proof}
Для $m=1$ - это следствие равенства
\EqRef{Gateaux differential of product, algebra}
\ShowEq{Gateaux derivative of f(x)x, 1, algebra}
Допустим, \EqRef{Gateaux derivative of f(x)x, algebra} справедливо
для $m-1$. Тогда
\ShowEq{Gateaux derivative of f(x)x, m-1, algebra}
Пользуясь равенствами
\EqRef{Gateaux differential of product, algebra}
и \EqRef{Gateaux derivative, product over constant, algebra}
получим
\ShowEq{Gateaux derivative of f(x)x, m, algebra}
Равенства \EqRef{Gateaux derivative of f(x)x, algebra} и
\EqRef{Gateaux derivative of f(x)x, m, algebra}
отличаются только формой записи.
Теорема доказана.
\end{proof}
\fi

\begin{theorem}
\label{theorem: Gateaux derivative of pn is symmetric, m < n, algebra}
Производная Гато
\ShowEq{Gateaux derivative of pn is symmetric}
является симметричным многочленом по переменным $h_1$, ..., $h_m$.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Для доказательства теоремы мы рассмотрим алгебраические свойства
производной Гато и дадим эквивалентное определение.
Мы начнём с построения одночлена.
Для произвольного одночлена $p_n(x)$ мы построим симметричный
многочлен $r_n(x)$ согласно следующим правилам
\begin{itemize}
\item Если $p_1(x)=a_0xa_1$, то $r_1(x_1)=a_0x_1a_1$
\item Если $p_n(x)=p_{n-1}(x)a_n$, то
\[
r_n(x_1,...,x_n)=r_{n-1}(x_{[1},...,x_{n-1})x_{n]}a_n
\]
где квадратные скобки выражают симметризацию выражения
по переменным $x_1$, ..., $x_n$.
\end{itemize}
Очевидно, что
\[
p_n(x)=r_n(x_1,...,x_n)\ \ \ x_1=...=x_n=x
\]
Мы определим производную Гато порядка $k$ согласно правилу
\ShowEq{Gateaux derivative of monomial, algebraic definition, algebra}
Согласно построению многочлен $r_n(h_1,...,h_k,x_{k+1},...,x_n)$
симметричен по переменным $h_1$, ..., $h_k$, $x_{k+1}$, ..., $x_n$.
Следовательно, многочлен
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
симметричен по переменным $h_1$, ..., $h_k$.

При $k=1$ мы докажем, что определение
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
производной Гато совпадает с определением
\EqRef{Gateaux derivative of map, algebra}.

Для $n=1$, $r_1(h_1)=a_0h_1a_1$. Это выражение совпадает
с выражением производной Гато в теореме
\ref{theorem: Gateaux derivative, fx=axb, algebra}.

Пусть утверждение справедливо для $n-1$.
Справедливо равенство
\ShowEq{Gateaux derivative of monomial, n, algebra}
Положим $x_2=...=x_n=x$. 
Согласно предположению индукции, из равенств
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra},
\EqRef{Gateaux derivative of monomial, n, algebra}
следует
\ShowEq{Gateaux derivative of monomial, n1, algebra}

Согласно теореме
\ref{theorem: Gateaux derivative of f(x)x, algebra}
\ShowEq{Gateaux derivative of pn is symmetric, 1}
что доказывает равенство
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
для $k=1$.

Докажем теперь, что определение
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
производной Гато совпадает с определением
\EqRef{Gateaux derivative of Order n, algebra} для $k>1$.

Пусть равенство
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
верно для $k-1$.
Рассмотрим произвольное слагаемое многочлена $r_n(h_1,...,h_{k-1},x_k,...,x_n)$.
Отождествляя переменные $h_1$, ..., $h_{k-1}$
с элементами тела $D$, мы рассмотрим многочлен
\begin{equation}
R_{n-k}(x_k,...,x_n)=r_n(h_1,...,h_{k-1},x_k,...,x_n)
\EqLabel{reduced polynom, algebra}
\end{equation}
Положим $P_{n-k}(x)=R_{n-k}(x_k,...,x_n)$, $x_k=...=x_n=x$.
Следовательно
\ShowEq{Gateaux derivative of pn is symmetric, 2}
Согласно определению
\EqRef{Gateaux derivative of Order n, algebra}
производной Гато
\ShowEq{Gateaux derivative of Order n, 1, algebra}
Согласно определению производной Гато
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
\ShowEq{Gateaux derivative of monomial, algebraic definition, 1, algebra}
Согласно определению \EqRef{reduced polynom, algebra},
из равенства
\EqRef{Gateaux derivative of monomial, algebraic definition, 1, algebra}
следует
\begin{equation}
\partial P_{n-k}(x)(h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\EqLabel{Gateaux derivative of monomial, algebraic definition, 2, algebra}
\end{equation}
Из сравнения равенств \EqRef{Gateaux derivative of Order n, 1, algebra}
и \EqRef{Gateaux derivative of monomial, algebraic definition, 2, algebra}
следует
\[
\partial^k p_n(x)(h_1;...;h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\]
Следовательно равенсто
\EqRef{Gateaux derivative of monomial, algebraic definition, algebra}
верно для любых $k$ и $n$.

Утверждение теоремы доказано.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn = 0, algebra}
Для произвольного $n\ge 0$ справедливо равенство
\ShowEq{Gateaux derivative n1 of pn, algebra}
\ePrints{2010.05.23}
\end{theorem}
\begin{proof}
Так как $p_0(x)=a_0$, $a_0\in D$, то при $n=0$ теорема является следствием
теоремы \ref{theorem: Gateaux derivative of const, algebra}.
Пусть утверждение теоремы верно для $n-1$. Согласно теореме
\ref{theorem: Gateaux derivative of f(x)x, algebra}
при условии $f(x)=p_{n-1}(x)$ мы имеем
\begin{align*}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})
=&\partial^{n+1}(p_{n-1}(x)xa_n)(h_1;...;h_{n+1})
\\
=&\partial^{n+1} p_{n-1}(x)(h_1;...;h_m)xa_n
\\
+&\partial^n p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^n p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
Согласно предположению индукции все одночлены равны $0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn = 0, m < n, algebra}
Если $m<n$, то справедливо равенство
\ShowEq{m Gateaux derivative of polinom pn, algebra}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\[
\partial^0 p_1(0)=a_0xa_1=0
\]
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \ref{theorem: Gateaux derivative of f(x)x, algebra}
\begin{align*}
&\partial^m (p_{n-1}(x)xa_n)(h_1;...;h_m)
\\
=&\partial^m p_{n-1}(x)(h_1;...;h_m)xa_n
+\partial^{m-1} p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^{m-1} p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
Первое слагаемое равно $0$ так как $x=0$.
Так как $m-1<n-1$, то
остальные слагаемые равны $0$ согласно предположению индукции.
Утверждение теоремы доказано.
\end{proof}
\fi

Если $h_1=...=h_n=h$, то мы положим
\ShowEq{dfxh}
Эта запись не будет приводить к неоднозначности, так как по числу аргументов
ясно, о какой функции идёт речь.

\begin{theorem}
\label{theorem: n Gateaux derivative of polinom pn, algebra}
Для произвольного $n>0$ справедливо равенство
\ShowEq{n Gateaux derivative of polinom pn, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\ShowEq{n Gateaux derivative of polinom pn, 2, algebra}
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \ref{theorem: Gateaux derivative of f(x)x, algebra}
\ShowEq{n Gateaux derivative of polinom pn, 1, algebra}
Первое слагаемое равно $0$ согласно теореме
\ref{theorem: Gateaux derivative of pn = 0, algebra}.
Остальные $n$ слагаемых равны, и согласно предположению индукции
из равенства \EqRef{n Gateaux derivative of polinom pn, 1, algebra}
следует
\ShowEq{n Gateaux derivative of polinom pn, 3, algebra}
Следовательно, утверждение теоремы верно для любого $n$.
\end{proof}

Пусть $p(x)$ - многочлен степени $n$.\footnote{Я рассматриваю
формулу Тейлора для многочлена по аналогии с
построением формулы Тейлора в \citeBib{Fihtengolts: Calculus volume 1}, с. 246.}
\[
p(x)=p_0+p_{1i_1}(x)+...+p_{ni_n}(x)
\]
Мы предполагаем сумму по индексу $i_k$, который нумерует слагаемые
степени $k$.
Согласно теоремам \ref{theorem: Gateaux derivative of pn = 0, algebra},
\ref{theorem: Gateaux derivative of pn = 0, m < n, algebra},
\ref{theorem: n Gateaux derivative of polinom pn, algebra}
\ShowEq{Taylor polynomial 1, algebra}
Следовательно, мы можем записать
\ShowEq{Taylor polynomial 2, algebra}
Это представление многочлена называется
\AddIndex{формулой Тейлора для многочлена}{Taylor polynomial, algebra}.
Если рассмотреть замену переменных $x=y-y_0$, то рассмотренное построение
остаётся верным для многочлена
\[
p(y)=p_0+p_{1i_1}(y-y_0)+...+p_{ni_n}(y-y_0)
\]
откуда следует
\ShowEq{Taylor polynomial 3, algebra}
\fi

Предположим, что функция $f(x)$ в точке $x_0$ дифференцируема в смысле Гато
до любого порядка.\footnote{Я рассматриваю
построение ряда Тейлора по аналогии с
построением ряда Тейлора в \citeBib{Fihtengolts: Calculus volume 1}, с. 248, 249.}

\begin{theorem}
\label{theorem: n Gateaux derivative equal 0, algebra}
Если для функции $f(x)$ выполняется условие
\ShowEq{n Gateaux derivatives of function, algebra}
то при $t\rightarrow 0$ выражение $f(x+th)$ является бесконечно малой порядка
выше $n$ по сравнению с $t$
\[
f(x_0+th)=o(t^n)
\]
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
При $n=1$ это утверждение следует из равенства
\EqRef{Gateaux differential of map, t, algebra}.

Пусть утверждение справедливо для $n-1$.
Для отображения
\ShowEq{n Gateaux derivative equal 0, 1, algebra}
выполняется условие
\ShowEq{n Gateaux derivative equal 0, 2, algebra}
Согласно предположению индукции
\[
f_1(x_0+th)=o(t^{n-1})
\]
Тогда равенство
\EqRef{Gateaux differential, representation in algebra}
примет вид
\[
o(t^{n-1})=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}f(x+th))
\]
Следовательно,
\[
f(x+th)=o(t^n)
\]
\end{proof}
\fi

Составим многочлен
\ShowEq{Taylor polynomial, f(x), algebra}
Согласно теореме \ref{theorem: n Gateaux derivative equal 0, algebra}
\[
f(x_0+t(x-x_0))-p(x_0+t(x-x_0))=o(t^n)
\]
Следовательно, полином $p(x)$ является хорошей апроксимацией отображения $f(x)$.

Если отображение $f(x)$ имеет производную Гато любого порядка, то переходя к пределу
$n\rightarrow\infty$, мы получим разложение в ряд
\ShowEq{Taylor series, f(x), algebra}
который называется \AddIndex{рядом Тейлора}{Taylor series, algebra}.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
{\bf Интеграл}
\fi
\Section{Интеграл}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
Понятие интеграла имеет разные аспекты. В этом разделе мы рассмотрим
интегрирование, как операцию, обратную дифференцированию.
По сути дела, мы рассмотрим процедуру решения обыкновенного дифференциального
уравнения
\ShowEq{differential equation, algebra}

\begin{example}
Я начну с примера дифференциального уравнения над полем действительных чисел.
\begin{equation}
\EqLabel{differential equation y=xx, 1, real number}
y'=3x^2
\end{equation}
\begin{equation}
\EqLabel{differential equation y=xx, initial, real number}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Последовательно дифференцируя равенство
\EqRef{differential equation y=xx, 1, real number},
мы получаем цепочку уравнений
\begin{align}
\EqLabel{differential equation y=xx, 2, real number}
y''&=6x
\\
\EqLabel{differential equation y=xx, 3, real number}
y'''&=6
\\
\EqLabel{differential equation y=xx, 4, real number}
y^{(n)}&=0&n&>3
\end{align}
Из уравнений
\EqRef{differential equation y=xx, 1, real number},
\EqRef{differential equation y=xx, initial, real number},
\EqRef{differential equation y=xx, 2, real number},
\EqRef{differential equation y=xx, 3, real number},
\EqRef{differential equation y=xx, 4, real number}
следует разложение в ряд Тейлора
\[
y=x^3
\]
\qed
\end{example}

\begin{example}
\fi
Рассмотрим аналогичное дифференциальное уравнение над алгеброй
\ShowEq{differential equation y=xx, algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
Последовательно дифференцируя равенство
\EqRef{differential equation y=xx, 1, algebra},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, 234, algebra}
Из уравнений
\EqRef{differential equation y=xx, 1, algebra},
\EqRef{differential equation y=xx, initial, algebra},
\EqRef{differential equation y=xx, 2, algebra},
\EqRef{differential equation y=xx, 3, algebra},
\EqRef{differential equation y=xx, 4, algebra}
следует разложение в ряд Тейлора
\[
y=x^3
\]
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\else
\qed
\end{example}
\fi

\begin{remark}
Я записываю  следующие равенства для того,
чтобы показать как работает производная. 
\ShowEq{differential equation y=xx, algebra, 1}
\qed
\end{remark}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{remark}
Дифференциальное уравнение
\ShowEq{differential equation y=xx, a, algebra}
так же приводит к решению $y=x^3$. Очевидно, что это
отображение не удовлетворяет дифференциальному уравнению.
Однако, вопреки теореме
\ref{theorem: Gateaux derivative of pn is symmetric, m < n, algebra}
вторая производная не
является симметричным многочленом. Это говорит о том,
что уравнение \EqRef{differential equation y=xx, 1, a, algebra}
не имеет решений.
\qed
\end{remark}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\begin{example}
Очевидно, если функция удовлетворяет дифференциальному уравнению
\ShowEq{differential equation, additive function, algebra}
то вторая производная Гато
\ShowEq{differential equation, additive function, 1, algebra}
Следовательно, если задано начальное условие $y(0)=0$,
то дифференциальное уравнение
\EqRef{differential equation, additive function, algebra} имеет решение
\ShowEq{differential equation, additive function, solution, algebra}
\qed
\end{example}

\Section{Экспонента}

В этом разделе мы рассмотрим одну из возможных моделей
построения экспоненты.

В поле мы можем определить экспоненту как решение дифференциального
уравнения
\ShowEq{exponent over field}
Очевидно, что мы не можем записать подобное уравнения для тела.
Однако мы можем воспользоваться равенством
\ShowEq{derivative over field}
Из уравнений
\EqRef{exponent over field}, \EqRef{derivative over field}
следует
\ShowEq{exponent derivative over field}
Это уравнение уже ближе к нашей цели,
однако остаётся открытым вопрос в каком порядке
мы должны перемножать $y$ и $h$.
Что бы ответить на этот вопрос, мы изменим запись уравнения
\else
\newpage
Рассмотрим уравнение
\fi
\ShowEq{exponent derivative over division ring}
Следовательно, наша задача - решить дифференциальное уравнение
\EqRef{exponent derivative over division ring}
при начальном условии $y(0)=1$.

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
Для формулировки и доказательства теоремы
\ref{theorem: exponent derivative n over division ring}
я введу следующее обозначение.
Пусть
\ShowEq{exponent derivative, transposition n}
перестановка кортежа переменных
\ShowEq{exponent transposition tuple 1}
Обозначим $p_{\sigma}(h_i)$ позицию, которую занимает
переменная $h_i$ в кортеже
\ShowEq{exponent transposition tuple 2}
Например, если перестановка $\sigma$ имеет вид
\ShowEq{exponent transposition tuple 3}
то следующие кортежи равны
\ShowEq{exponent transposition tuple 4}

\begin{theorem}
\label{theorem: exponent derivative n over division ring}
Производная Гато порядка $n$ функции $y$, удовлетворяющей дифференциальному уравнению
\EqRef{exponent derivative over division ring}
имеет вид
\ShowEq{exponent derivative n over division ring}
где сумма выполнена по перестановкам
\ShowEq{exponent derivative, transposition n}
множества переменных $y$, $h_1$, ..., $h_n$.
Перестановка $\sigma$ обладает следующими свойствами
\begin{enumerate}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$p_{\sigma}(h_i)$ располагается в произведении
\EqRef{exponent derivative n over division ring}
левее $p_{\sigma}(h_j)$ и $p_{\sigma}(h_j)$ располагается
левее $p_{\sigma}(y)$, то $i<j$.
\label{enumerate: exponent derivative, transposition n, left}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$p_{\sigma}(h_i)$ располагается в произведении
\EqRef{exponent derivative n over division ring}
правее $p_{\sigma}(h_j)$ и $p_{\sigma}(h_j)$ располагается
правее $p_{\sigma}(y)$, то $i>j$.
\label{enumerate: exponent derivative, transposition n, right}
\end{enumerate}
\end{theorem}
\begin{proof}
Мы докажем это утверждение индукцией.
Для $n=1$ утверждение верно, так как это дифференциальное уравнение
\EqRef{exponent derivative over division ring}.
Пусть утверждение верно для $n=k-1$.
Следовательно
\ShowEq{exponent derivative n=k-1 over division ring}
где сумма выполнена по перестановкам
\ShowEq{exponent derivative, transposition n=k-1}
множества переменных $y$, $h_1$, ..., $h_{k-1}$.
Перестановка $\sigma$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
Согласно определению
\EqRef{Gateaux derivative of Order n, algebra}
производная Гато` порядка $k$ имеет вид
\ShowEq{exponent derivative n=k over division ring, 1}
Из равенств
\EqRef{exponent derivative over division ring},
\EqRef{exponent derivative n=k over division ring, 1}
следует
\ShowEq{exponent derivative n=k over division ring, 2}
Нетрудно видеть, что произвольная перестановка $\sigma$
из суммы
\EqRef{exponent derivative n=k over division ring, 2}
порождает две перестановки
\ShowEq{exponent derivative, transposition n=k}
Из \EqRef{exponent derivative n=k over division ring, 2}
и \EqRef{exponent derivative, transposition n=k}
следует
\ShowEq{exponent derivative n=k over division ring, 3}
В выражении
\EqRef{exponent derivative n=k over division ring, 3}
$p_{\tau_1}(h_k)$ записано непосредственно перед $p_{\tau_1}(y)$.
Так как $k$ - самое большое значение индекса,
то перестановка $\tau_1$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
В выражении
\EqRef{exponent derivative n=k over division ring, 3}
$p_{\tau_2}(h_k)$ записано непосредственно после $p_{\tau_2}(y)$.
Так как $k$ - самое большое значение индекса,
то перестановка $\tau_2$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.

Нам осталось показать, что в выражении
\EqRef{exponent derivative n=k over division ring, 3}
перечислены все перестановки $\tau$, удовлетворяющие условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
Так как $k$ - самый большой индекс, то согласно условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме, $\tau(h_k)$
записано непосредственно перед или непосредственно после $\tau(y)$.
Следовательно, любая перестановка $\tau$ имеет
либо вид $\tau_1$, либо вид $\tau_2$.
Пользуясь равенством
\EqRef{exponent derivative, transposition n=k},
мы можем для заданной перестановки $\tau$ найти соответствующую
перестановку $\sigma$.
Следовательно, утверждение теоремы верно для $n=k$.
Теорема доказана.
\end{proof}
\fi

\begin{theorem}
Решением дифференциального уравнения
\EqRef{exponent derivative over division ring}
при начальном условии $y(0)=1$
является экспонента
\ShowEq{exponent over division ring}
которая имеет следующее разложение в ряд Тейлора
\ShowEq{exponent Taylor series over division ring}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Производная Гато порядка $n$ содержит $2^n$ слагаемых.
Действительно, производная Гато порядка $1$ содержит $2$ слагаемых,
и каждое дифференцирование увеличивает число слагаемых вдвое.
Из начального условия $y(0)=1$ и теоремы
\ref{theorem: exponent derivative n over division ring}
следует, что производная Гато порядка $n$ искомого решения имеет вид
\ShowEq{exponent derivative n over division ring, x=0}
Из равенства
\EqRef{exponent derivative n over division ring, x=0}
следует разложение
\EqRef{exponent Taylor series over division ring}.
в ряд Тейлора.
\end{proof}
\fi

\begin{theorem}
\label{theorem: exponent of sum}
Равенство
\ShowEq{exponent of sum}
справедливо тогда и только тогда, когда
\ShowEq{exponent of sum, 1}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть ряды Тейлора
\ShowEq{exponent a b a+b}
Перемножим выражения
\EqRef{exponent a} и \EqRef{exponent b}.
Сумма одночленов порядка $3$ имеет вид
\ShowEq{exponent ab 3}
и не совпадает, вообще говоря, с выражением
\ShowEq{exponent a+b 3}
Доказательство утверждения, что
\EqRef{exponent of sum} следует из \EqRef{exponent of sum, 1}
тривиально.
\end{proof}

Смысл теоремы \ref{theorem: exponent of sum}
становится яснее, если мы вспомним, что существует две
модели построения экспоненты. Первая модель - это
решение дифференциального уравнения
\EqRef{exponent derivative over division ring}.
Вторая - это изучение однопараметрической группы преобразований.
В случае поля обе модели приводят к одной и той же функции.
Я не могу этого утверждать сейчас в общем случае. Это вопрос отдельного
исследования. Но если вспомнить, что кватернион является аналогом
преобразования трёхмерного пространства, то утверждение теоремы
становится очевидным.
\fi


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {$(^a_b)$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb%
   {минор}%
   {A from b a}%
\Symb%
   {минор}%
   {A from columns T}%
\Symb%
   {минор}%
   {A from rows S}%
\Symb%
   {минор}%
   {A without column a}%
\Symb%
   {минор}%
   {A without columns T}%
\Symb%
   {минор}%
   {A without row b}%
\Symb%
   {минор}%
   {A without rows S}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 1}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 2}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $R$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $R$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения $\Vector{A}$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {CR linear combination in A module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение переменной $v^i$}%
   {partial linear map of variable}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $\Vector a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество $A$\Hyph линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set A linear maps, module}%
\Symb%
   {множество линейных отображений тела $D_1$ в тело $D_2$}%
   {set linear maps, division ring}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
\Symb%
   {тензорное произведение представлений}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {структурные константы алгебры $A$ над кольцом $D$}%
   {structural constants of algebra}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли}%
   {basis vector of representation of Lie group}%
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {координаты базового вектора представления группы Ли}%
   {basis vector of representation of Lie group, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of map, algebra}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ алгебры}%
   {component of Gateaux derivative of Second Order, algebra}%
\Symb%
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, algebra}%
\Symb%
   {производная Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Symb%
   {производная Гато отображения $f$ алгебры}%
   {Gateaux derivative of map, fraction, algebra}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, algebra}%
\Symb%
   {производная Гато второго порядка отображения $\Vector f$}%
   {Gateaux derivative of Second Order, D vector space}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$ алгебры}%
   {Gateaux differential of map, algebra}%
\Symb%
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ алгебры}%
   {Gateaux differential of Second Order, algebra}%
\Symb%
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ тела}%
   {Gateaux differential of Second Order, division ring}%
\Symb%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb%
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Symb%
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато отображения $f$}%
   {standard component of Gateaux derivative, algebra}%
\Symb%
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 1}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 2}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения ассоциативной алгебры}%
   {component of polylinear map, associative algebra}%
\Symb%
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма отображения в $D$\Hyph алгебру}%
   {norm of map, algebra}%
\Symb%
   {норма отображения $f$  тела}%
   {norm of map, division ring}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная $F$\Hyph компонента линейного отображения $f$ }%
   {standard component of linear map, division ring}%
\Symb%
   {стандартная компонента полилинейного отображения в ассоциативную алгебру}%
   {standard component of polylinear map, associative algebra}%
\Symb%
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator I of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор отображения $f$}%
   {vector of mapping}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения $D$\Hyph векторного пространства}%
   {kernel of linear map, D vector space}%
\Symb%
   {ядро линейного отображения тела}%
   {kernel of linear map, division ring}%

\SetIndexSpace%L%0
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности в нормированном кольце}%
   {limit of sequence, normed ring}%
\Symb%
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Symb%
   {предел последовательности в нормированном кольце}%
   {limit of sequence, valued ring}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {множество \Acr линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%
   {\rcd векторное пространство \drc линейных отображений \drc векторного пространства $\Vector V$ в \drc векторное пространство $\Vector W$}%
   {set drc linear maps, drc vector space}%
\Symb%
   {множество линейных отображений алгебры $A_1$ в алгебру $A_2$}%
   {set linear mappings, algebra}%
\Symb%
   {множество линейных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set linear maps, D vector space}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество $n$\hyph линейных отображений алгебры $A$ в модуль $S$}%
   {set polylinear mappings An, algebra}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$  в модуль $S$}%
   {set polylinear mappings, algebra}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {\drc векторное пространство \rcd линейных отображений \rcd векторного пространства $\Vector{V}$ в \rcd векторное пространство $\Vector{W}$}%
   {set rcd linear maps, rcd vector space}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований универсальной алгебры $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $R$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр отображения $f$}%
   {scalar of mapping}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $R$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex


==> Tensor.Algebra.Russian.tex <==
%auto-ignore
\input{\FilePrefix Tensor.Algebra.Eq}

%\chapter{Тензорное произведение}

\ePrints{1011.3102}
\ifx\Semafor\ValueOff
\Section{Тензорное произведение алгебр}
\else
\section{Тензорное произведение алгебр}
\fi
\label{Section: Tensor Product of Algebras}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOff
\begin{definition}
\label{definition: tensor product of algebras}
Пусть $A_1$, ..., $A_n$ -
свободные алгебры над  коммутативным кольцом $D$.\footnote{Я определяю
тензорное произведение $D$\Hyph алгебр
по аналогии с определением в \citeBib{Serge Lang}, с. 456 - 458.
\ePrints{Calculus.Paper}
\Items{1011.3102}
\ifx\Semafor\ValueOn
Этот
подраздел написан на основе раздела
\xRef{8433-5163}{Section: Tensor Product of Algebras}.
\fi
}
Рассмотрим категорию $\mathcal A$ объектами которой являются
полилинейные над коммутативным кольцом $D$ отображения
\ShowEq{polylinear mappings category}
где $S_1$, $S_2$ - модули над кольцом $D$.
Мы определим морфизм $f\rightarrow g$
как линейное над коммутативным кольцом $D$ отображение $h:S_1\rightarrow S_2$,
для которого коммутативна диаграмма
\ShowEq{polylinear mappings category, diagram}
Универсальный объект
\ShowEq{tensor product of algebras}
категории $\mathcal A$
называется \AddIndex{тензорным произведением алгебр $A_1$, ..., $A_n$}
{tensor product of algebras}.
\qed
\end{definition}

\begin{definition}
\label{definition: tensor power of algebra}
Тензорное произведение
\ShowEq{tensor power of algebra}
называется
\AddIndex{тензорной степенью алгебры}{tensor power of algebra} $A$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: tensor product of algebras is module}
Тензорное произведение алгебр существует.
\end{theorem}
\begin{proof}
Пусть $M$ - модуль над кольцом $D$, порождённый
произведением $\Times$
$D$\Hyph алгебр $A_1$, ..., $A_n$.
Инъекция
\ShowEq{map i, algebra, tensor product, 1}
определена по правилу
\ShowEq{map i, algebra, tensor product}
Пусть $N\subset M$ - подмодуль, порождённый элементами вида
\ShowEq{kernel, algebra, tensor product}
где $d_i\in A_i$, $c_i\in A_i$, $a\in D$.
Пусть
\[
j:M\rightarrow M/N
\]
каноническое отображение на фактормодуль.
Рассмотрим коммутативную диаграмму
\ShowEq{diagram top, algebra, tensor product}
Поскольку элементы \EqRef{kernel 1, algebra, tensor product}
и \EqRef{kernel 2, algebra, tensor product}
принадлежат ядру линейного отображения $j$,
то из равенства
\EqRef{map i, algebra, tensor product}
следует
\ShowEq{f, algebra, tensor product}
Из равенств \EqRef{f 1, algebra, tensor product}
и \EqRef{f 2, algebra, tensor product}
следует, что отображение $f$ полилинейно над кольцом $D$.
Поскольку $M$ - модуль с базисом
$\Times$, то, согласно теореме \citeBib{Serge Lang}-1
на с. 104,
для любого модуля $V$ и любого
полилинейного над $D$ отображения
\ShowEq{diagram bottom, 1, algebra, tensor product}
существует единственный гомоморфизм $k:M\rightarrow V$,
для которого коммутативна следующая диаграмма
\ShowEq{diagram bottom, algebra, tensor product}
Так как $g$ - полилинейно над $D$, то
\ShowEq{ker k subseteq N}
Согласно утверждению 
на с. \citeBib{Serge Lang}-94,
отображение $j$ универсально в категории гомоморфизмов
векторного пространства $M$,
ядро которых содержит $N$.
Следовательно, определён гомоморфизм
\[
h:M/N\rightarrow V
\]
для которого коммутативна диаграмма
\begin{equation}
\EqLabel{diagram right, algebra, tensor product}
\xymatrix{
&M/N\ar[dd]^h
\\
M\ar[dr]^k\ar[ur]_j
\\
&V
}
\end{equation}
Объединяя диаграммы
\EqRef{diagram top, algebra, tensor product},
\EqRef{diagram bottom, algebra, tensor product},
\EqRef{diagram right, algebra, tensor product},
получим коммутативную диаграмму
\ShowEq{diagram, algebra, tensor product}
Так как $\mathrm{Im}f$ порождает $M/N$,
то отображение $h$ однозначно определено.
\end{proof}

Согласно доказательству теоремы
\ref{theorem: tensor product of algebras is module}
\[A_1\otimes...\otimes A_n=M/N\]
Для $d_i\in A_i$ будем записывать
\ShowEq{map j, algebra, tensor product}

\begin{theorem}
\label{theorem: tensor product and polylinear mapping}
Пусть $A_1$, ..., $A_n$ -
алгебры над коммутативным кольцом $D$.
Пусть
\ShowEq{map f, 1, algebra, tensor product}
полилинейное отображение, определённое равенством
\ShowEq{map f, algebra, tensor product}
Пусть
\ShowEq{map g, algebra, tensor product}
полилинейное отображение в $D$\Hyph модуль $V$.
Существует $D$\Hyph линейное отображение
\ShowEq{map h, algebra, tensor product}
такое, что диаграмма
\ShowEq{map gh, algebra, tensor product}
коммутативна.
\end{theorem}
\begin{proof}
Равенство
\EqRef{map f, algebra, tensor product}
следует
из равенств
\EqRef{map i, algebra, tensor product} и
\EqRef{map j, algebra, tensor product}.
Существование отображения $h$ следует из определения
\ref{definition: tensor product of algebras}
и построений, выполненных при доказательстве теоремы
\ref{theorem: tensor product of algebras is module}.
\end{proof}

Равенства \EqRef{f 1, algebra, tensor product}
и \EqRef{f 2, algebra, tensor product}
можно записать в виде
\ShowEq{tensors, algebra, tensor product}

\begin{theorem}
\label{theorem: tensor product and product in algebra}
Пусть $A$ -
алгебра над коммутативным кольцом $D$.
Существует линейное отображение
\ShowEq{tensor product and product in algebra}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: tensor product and polylinear mapping}
и определения
\ref{definition: algebra over ring}.
\end{proof}
\else
\newpage
Для $a_i\in A_i$, $i=1$, ..., $n$,
$a_1\otimes...\otimes a_n\in A_1\otimes...\otimes A_n$.
Согласно определению
\ShowEq{tensors, algebra, tensor product}

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{remark}
\label{remark: representation of tensor, ring}
Представление тензора в виде
\ShowEq{tensor representation, algebra}
неоднозначно.
Если $r\in D$, то
\[
(d_1 r)
\otimes
d_2
=d_1
\otimes
(rd_2 )
\]
Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
К числу допустимых преобразований относится
\begin{align*}
&d_1
\otimes
d_2
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2+c_2)
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2)
+d_1
\otimes
c_2
+c_1
\otimes
c_2
\\
=&d_1
\otimes
(d_2-c_2)
+(d_1
+c_1)
\otimes
c_2
\end{align*}
\qed
\end{remark}
\fi

\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\newpage
\fi
\begin{theorem}
\label{theorem: standard component of tensor, algebra}
Тензорное произведение $\Tensor A$ свободных
конечномерных алгебр
$A_1$, ..., $A_n$
над коммутативным кольцом $D$ является свободной
конечномерной алгеброй.

Пусть
\ShowEq{tensor product of algebras, basis i}
- базис алгебры $A_i$ над кольцом $D$.
Произвольный тензор $a\in\Tensor A$ можно представить в виде
\ShowEq{tensor canonical representation, algebra}
%Выражение \EqRef{tensor canonical representation, algebra}
%определенно однозначно с точностью до выбора базиса.
Мы будем называть выражение
$\ShowSymbol{standard component of tensor, algebra}$
\AddIndex{стандартной компонентой тензора}
{standard component of tensor, algebra}.
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\Items{1011.3102}
\ifx\Semafor\ValueOn
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: standard component of tensor, algebra}.
\else
Алгебры
$A_1$, ..., $A_n$
являются модулями над кольцом $D$.
Согласно теореме
\ref{theorem: tensor product of algebras is module},
$\Tensor A$ является модулем. 

Вектор $a_i\in A_i$ имеет разложение
\ShowEq{expansion i relative basis}
относительно базиса $\Basis e_i$.
Из равенств
\EqRef{tensors 1, algebra, tensor product},
\EqRef{tensors 2, algebra, tensor product}
следует
\ShowEq{expansion i relative basis, 1}
Так как множество тензоров $\Tensor a$
является множеством образующих модуля $\Tensor A$,
то тензор
$a\in\Tensor A$
можно записать в виде
\ShowEq{tensor canonical representation 1, algebra}
где
\ShowEq{tensor canonical representation 2, algebra}
Положим
\ShowEq{tensor canonical representation 3, algebra}
Тогда равенство \EqRef{tensor canonical representation 1, algebra}
примет вид
\EqRef{tensor canonical representation, algebra}.

Следовательно, множество тензоров $\TensorBasis i$
является множеством образующих модуля $\Tensor A$.
Так как размерность модуля $A_i$, $i=1$, ..., $n$, конечна,
то конечно множество тензоров $\TensorBasis i$.
Следовательно, множество тензоров $\TensorBasis i$
содержит базис модуля $\Tensor A$, и модуль $\Tensor A$
является свободным модулем над кольцом $D$.

Мы определим произведение тензоров типа $\Tensor a$ покомпонентно
\ShowEq{product of tensors, algebra, tensor product}
В частности, если для любого $i$, $i=1$, ..., $n$,
$a_i\in A_i$ имеет обратный,
то тензор
\ShowEq{inverse tensor, algebra, 1}
имеет обратный
\ShowEq{inverse tensor, algebra, 2}

Определение произведения
\EqRef{product of tensors, algebra, tensor product}
согласовано с равенством
\EqRef{tensors 2, algebra, tensor product}
так как
\ShowEq{product of tensors, algebra, tensor product, 1}
Из равенства
\EqRef{tensors 1, algebra, tensor product}
следует дистрибутивность умножения по отношению к сложению
\ShowEq{product of tensors, algebra, tensor product, 2}
Равенство
\EqRef{product of tensors, algebra, tensor product, 2}
позволяет определить произведение для любых тензоров $a$, $b$.
\fi
\end{proof}

\ePrints{Calculus.Paper}
\Items{1011.3102}
\ifx\Semafor\ValueOff
\begin{remark}
\label{remark: tensor product of algebras}
Согласно замечанию
\ref{remark: opposite algebra},
мы можем определить различные структуры алгебры
в тензорном произведении алгебр.
Например, алгебры $A_1\otimes A_2$,
$A_1\otimes A_2^*$, $A_1^*\otimes A_2$
определены на одном и том же модуле.
\qed
\end{remark}
\fi
\fi

\ePrints{Calculus.Paper}
\Items{1011.3102}
\ifx\Semafor\ValueOff
\begin{theorem}
Пусть $\Basis e_i$ - базис алгебры $A_i$ над кольцом $D$.
Пусть $B_{i\cdot}{}^{\gi j}_{\gi{kl}}$ -
структурные константы алгебры $A_i$ относительно базиса $\Basis e_i$.
Структурные константы тензорного произведение $\Tensor A$
относительно базиса $\TensorBasis i$ имеют вид
\ShowEq{structural constants tensor algebra}
\ePrints{2010.05.23}
\ifx\Semafor\ValueOn
\qed
\end{theorem}
\newpage
\else
\end{theorem}
\begin{proof}
Непосредственное перемножение тензоров
$\TensorBasis i$ имеет вид
\ShowEq{structural constants tensor algebra, proof, 1}
Согласно определению структурных констант
\ShowEq{structural constants tensor algebra, proof, 2}
Равенство
\EqRef{structural constants tensor algebra}
следует из сравнения
\EqRef{structural constants tensor algebra, proof, 1},
\EqRef{structural constants tensor algebra, proof, 2}.

Из цепочки равенств
\ShowEq{structural constants tensor algebra, proof, 3}
следует, что определение произведения
\EqRef{structural constants tensor algebra, proof, 2}
со структурными константами
\EqRef{structural constants tensor algebra}
согласовано с определением произведения
\EqRef{product of tensors, algebra, tensor product}.
\end{proof}

\begin{theorem}
Для тензоров $a$, $b\in\Tensor A$
стандартные компоненты произведения удовлетворяют равенству
\ShowEq{standard components of product, tensor product}
\end{theorem}
\begin{proof}
Согласно определению
\ShowEq{standard components of product, tensor product, 1}
В тоже время
\ShowEq{standard components of product, tensor product, 2}
Равенство
\EqRef{standard components of product, tensor product}
следует из равенств
\EqRef{standard components of product, tensor product, 1},
\EqRef{standard components of product, tensor product, 2}.
\end{proof}

\begin{theorem}
Если алгебра $A_i$, $i=1$, ..., $n$, ассоциативна,
то тензорное произведение $\Tensor A$ - ассоциативная алгебра.
\end{theorem}
\begin{proof}
Поскольку
\ShowEq{tensor product, associative algebra, 1}
то
\ShowEq{tensor product, associative algebra, 2}
\end{proof}
\fi
\fi
